MAP's not dead yet: Uncovering true language model modes by conditioning away degeneracy

It has been widely observed that exact or approximate MAP (mode-seeking) decoding from natural language generation (NLG) models consistently leads to degenerate outputs (Holtzman et al., 2019; Stahlberg and Byrne, 2019). Prior work has attributed this behavior to either a fundamental and unavoidable inadequacy of modes in probabilistic models or weaknesses in language modeling. Contrastingly, we argue that degenerate modes can even occur in the absence of any modeling error, due to contamination of the training data. Specifically, we argue that mixing even a tiny amount of low-entropy noise with a population text distribution can cause the data distribution's mode to become degenerate. We therefore propose to apply MAP decoding to the model's true conditional distribution where the conditioning variable explicitly avoids specific degenerate behavior. Using exact search, we empirically verify that the length-conditional modes of machine translation models and language models are indeed more fluent and topical than their unconditional modes. For the first time, we also share many examples of exact modal sequences from these models, and from several variants of the LLaMA-7B model. Notably, we observe that various kinds of degenerate modes persist, even at the scale of LLaMA-7B. Although we cannot tractably address these degeneracies with exact search, we perform a classifier-based approximate search on LLaMA-7B, a model which was not trained for instruction following, and find that we are able to elicit reasonable outputs without any finetuning.

==> modes/beam_chapter.tex <==
\chapter{Approximate mode search with conditional beam search}\label{chapter:modes_beam}
\begin{comment}
Results:
- Beam search samples for NMT/ROC
    - Re-run with no marginal, running
- Beam search outputs for LLaMA
    - Get classifier probabilities for raw and modified beam search
        - Calculate average satisfaction before/after
        - Calculate after change in probability
    - Identify which data training/testing was done on
    - Figure out whether I used GPT-4 for irrelevance
- Show outputs for NMT, ROC, LLaMA

Training data:
    - ROC training was data free
    - MT data was news commentary
    - LLaMA data: Alpaca training, Dolly measurement

In paper:
    - Llama classifier improvement
    - MT guided search winrate
    - Roc guided search winrate
Done:
    - MT random samples
    - ROC random samples
Running:
- Beam size 20 ROC
Coded:
- Beam size 20 marian
- Beam size 20 ROC plot
 Beam size 20 marian plot
TODO:
    - LLama random samples

Outline:
- We've argued that MAP is probably bad due to a certain type of degeneracy, but we think that we can condition it out
- Furthermore, currently we get our desired behavior by destroying the distribution of the pretrained LM
- Conditional sampling is valuable but more explored so we leave it to future work
- Approximate search: How to do beam search
- Experiments on NMT and ROC verify that we're doing better search and getting outputs which are simultaneously higher likelihood \emph{and} higher quality
- Experiments on LLaMA are suboptimal in several ways, but we verify that we can get the degenerate outputs under control to some extent
\end{comment}
\section{Introduction}
In the previous two chapters we looked at the bad mode problem both in theory and with several actual models.
Chapter~\ref{chapter:modes_exact} showed that while all these models display the bad mode problem, conditioning on output length could get it under control for the MT model and story completion model.
The LLaMA model derivatives instead displayed a wider variety of issues, such as modes that repeated the prompt or consisted of a single \LaTeX{} fragment, on top of the empty mode issue.

The current way we force LLMs to give acceptable outputs is a combination of supervised finetuning (SFT), and reinforcement learning from human feedback (RLHF).
Both of these methods alter the model's output distribution to get it to output text that is more relevant, factual, non-toxic, etc.
The downside of these methods is that they don't include any incentive for the LM to maintain good coverage of the output space.

This is not just a theoretical problem: GPT-4, the best publicly available LLM at present, appears to put most of its output probability mass on just a few sequences.
When GPT-4 was given the input\footnote{On July 31, 2023, using a temperature of 1.} ``Write a haiku'' 20 times, the outputs had extremely low variation.
For example, 17 of the 20 outputs had the string ``whispers'' in them, and 10 mentioned the moon.

As we argued in Chapter~\ref{chapter:modes_theory}, at least part of what is happening is that our decoding methods don't appropriately handle various types of noise in our training data.
This means that if we want our inadequate decoding methods to produce high-quality results, we need to make sure the model we're using them on is \emph{extremely} unlikely to produce noisy outputs.
This is likely one of the pressures leading to the mode collapse described above.

While in this section we won't be tackling the problem of \emph{sampling} from models, we are still interested in the question of how much we can improve decoding while leaving the model fixed.
In the last chapter, all the models we ran exact MAP inference on showed degenerate modes.
However, the modes were often high-quality, and this was much more likely to be the case when we instead searched for an appropriate \emph{conditional mode}.
Encouraged by these results, we developed a variant of beam search to search for conditional modes, in the same way that ordinary beam search approximates search for the unconditional mode.

The rest of this chapter's contents are as follows.
In Section~\ref{sec:modesbeam_beam}, we derive \emph{conditional beam search}.
Section~\ref{sec:modesbeam_alternatives} discusses the connection between conditional beam search and existing methods for conditional sampling.
In Section~\ref{sec:modesbeam_length} we demonstrate that using conditional beam search while conditioning on length usually leads to higher-likelihood and more grammatical outputs of a desired length than merely constraining standard beam search does.

While the length constraint results support our hypotheses about the bad modes problem and the functionality of conditional beam, they aren't of much use for practical NLG applications.
In order to bridge this gap, in Section~\ref{sec:modesbeam_llama}, we apply conditional beam search to LLaMA-7B, despite the fact that beam search is usually seen as a poor choice for more open ended tasks.
We find that even using just 500 labeled examples, we're able to significantly improve the output compared to ordinary beam search.
These experiments support our repeated claim that while MAP may not be a good decoding method, MAP on the conditional distribution $\pmodel\left( x \given[\big] A(x) = a\right)$ can give good results.

\section{Conditional beam search}\label{sec:modesbeam_beam}
In this section, we'll discuss how to modify beam search to search for \emph{conditionally} high likelihood sequences, rather than the unconditional mode.
Our method is very similar to FUDGE\citep{fudge}, but there are some additional details necessary to support doing beam search instead of sampling.
We discuss the relationship of our method to theirs in Section~\ref{sec:modesbeam_alternatives}, as well as some possible alternative methods.

Beam search is a heuristic method for finding outputs that an autoregressive model assigns a high likelihood to (usually conditional on some other text such as a sentence to be translated).
As we've discussed in the previous two chapters, disagreement between the actual quality of an output and the likelihood our model assigns it is a well-known problem (see the discussion of prior work in Chapter~\ref{chapter:modes_theory}).

%When beam search is introduced, it's usually described as trading off compute cost and quality, since in the limit of increasing beam size, beam search will eventually find the exact mode.
%This isn't true in practice, and using a beam size which is not too big and not too small is usually best.

In standard beam search, we're doing approximate search for the unconditional mode of the model's output distribution.
Beam search assigns each partial hypotheses of length $t$ a score $S(x_{1:t})$.
The score is just its log-likelihood under $\pmodel$ calculated using the chain rule of probability:\footnote{For a conditional task like MT, the probability would instead be $\pmodel\left(x_i \given[\big] x_{<i}, s \right)$ for a source sequence $s$. For brevity (and to keep notation uniform), we'll leave out the dependence on the conditioning information.}
\begin{equation}\label{eq:beam}
    S(x_{1:t}) = \sum\limits_{i=1}^t \log \left(\pmodel(x_i | x_{<i})\right)
\end{equation}
If $x_{1:t}$ is a complete sequence\footnote{I.e., it ends in the end-of-sentence token}, this score is exactly its log-probability under the model.

Instead of searching for the argmax of $\pmodel(x)$ (the unconditional mode), we want to change this to the argmax of $\pmodel(x | A(x) = a)$ for some attribute $a$ (the conditional mode).
To start with, we can replace the marginal distribution Equation~\ref{eq:beam} with one that conditions on the event that $A(x) = a$:
\begin{equation}\label{eq:cond_beam}
    S'(x_{1:t}, a) = \sum\limits_{i=1}^t \log \left(\pmodel(x_i | x_{<i}, A(x) = a)\right)
\end{equation}
This can be simplified by applying Bayes' rule to any term in the sum:
\begin{equation}\label{eq:bayes}
    \pmodel\left(x_i \given[\big] x_{<i}, A(x) = a\right) = \frac{
        \pmodel\left(A(x) = a \given[\big] x_i, x_{<i}\right) \pmodel\left(x_i \given[\big] x_{<i}\right)
    }{
        \pmodel\left(A(x) = a \given[\big] x_{<i}\right)
    }
\end{equation}
This shows that the denominator in $i$th summand in Equation~\ref{eq:cond_beam} is the same as the numerator in the $i-1$th summand, so part of the sum telescopes:
\begin{align*}
S'(x_{1:t}, a) &= -\log\pmodel\left(A(x) = a\right) + \left(
    \sum\limits_{i=1}^t \log \pmodel\left(x_i \given[\big] x_{<i}\right)
\right) + \log\pmodel\left(A(x) = a \given[\big] x_{1:t}\right)\\
&= -\log\pmodel\left(A(x) = a) + S(x_{1:t}\right) + \log\pmodel\left(A(x) = a \given[\big] x_{1:t}\right)\\
\end{align*}
The first term is just the marginal log-likelihood of the attribute occurring, but it doesn't differ between hypotheses.
Since we only care about the relative value of the score between different hypotheses, we discard it to get our final conditional score:
\begin{align*}
    S_\text{cond}(x_{1:t}, a) &= S(x_{1:t}) + \log\pmodel\left(A(x) = a \given[\big] x_{1:t}\right)\\
\end{align*}
So to do conditional beam search, we just need to add one term to the normal beam search score.
To clear up a possible point of confusion, $\log\pmodel(A(x) = a | x_{1:t}$ is \emph{not} the probability that $x_{1:t}$ has the desired attribute.
It is the probability that the final output will have that attribute, conditional on a prefix of $x_{1:t}$.
The problem is that it's intractable to compute, since we'd need to marginalize over all sequences which have $x_{1:t}$ as their first $t$ tokens.

To avoid this, we will train a classifier to estimate this probability, calling the predicted probability $\pclf\left(A(x) = a \given[\big] x_{1:t}\right)$.
The important thing is that we're trying to specifically predict the probability of a \emph{model output} having the attribute, which means the classifier should be trained on model outputs rather than naturally occuring text.
Substituting in the classifier prediction gives us a score we can actually use for decoding:
\begin{equation}\label{eq:beam_final}
    S_\text{clf}(x_{1:t}, a) = S(x_{1:t}) + \log\pclf\left(A(x) = a \given x_{1:t}\right)\\
\end{equation}
Notice that the probability of the attribute being satisfied doesn't need to be accumulated across timesteps.
This means that $\pclf$ is only used for selecting new hypotheses, but doesn't contribute to the running beam score.
If we didn't take advantage of the telescoping simplification, the value of $\pclf(A(x) = a | x_{<t}$ calculated by marginalizing $\pclf(A(x) = a | x_{1:t})$ (i.e., predicted on step $t$) will be different from the value that was predicted on step $t-1$, since the $\pclf$ may not be temporally consistent.
Using the simplification above lets us avoid accumulating error in the scores.

The last detail to specify is that we only calculate $\log\pclf(A(x) = a | x_{1:t})$ for the $k$ tokens with the highest likelihood, for computational efficiency.\footnote{The reason for doing this is discussed more in Section~\ref{sec:modesbeam_alternatives}.}.
The full method is formally shown in Algorithm~\ref{alg:beam_cond}.

\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}
\begin{algorithm}
\caption{Conditional beam search. This searches for an output with a sequence $x$ with a high value of $\pmodel(x, A(x) = a)$ for some target attribute $a$. In order to execute this efficiently one needs to efficiently compute $\pmodel$ and $\pclf$ to avoid recomputation, rather than just fully re-executing them as the pseudocode implies. How this is done will depend on the model architectures, see Section~\ref{sec:modesbeam_alternatives} for discussion.}\label{alg:beam_cond}

 \hspace*{\algorithmicindent}\textbf{Input:} \\
 \hspace*{\algorithmicindent} $\: a$: The target attribute value\\
 \hspace*{\algorithmicindent} $\: V$: Vocabulary\\
 \hspace*{\algorithmicindent} $\: B > 0$: Beam size\\
 \hspace*{\algorithmicindent} $\: L > 0$: Maximum output length\\
 \hspace*{\algorithmicindent} $\: k > 0$: Number of continuations to score for each hypothesis.\\
 \hspace*{\algorithmicindent} $\: \alpha > 0$: Optional attribute weight.\\
 \hspace*{\algorithmicindent}\textbf{Output:} A string in $V*$ with length at most $L$
\begin{algorithmic}[1]
\State $X[b] = \epsilon$ for $b \in {1, \dots, B}$ \qquad\{Initialize all hypotheses to the empty sequence\}
\State $S \gets [0, -\infty, -\infty, \dots, -\infty]$ \qquad\{A length $B$ array of cumulative scores, only $S[0]$ is initially finite.\}
\State $t \gets 1$
\While{Any hypothesis $X[i]$ on the beam is not complete AND $t \le L$}
    \State Init empty $b \times k$ array $U_t$ \qquad\{Unconditional scores\}
    \State Init empty $b \times k$ array $C_t$ \qquad\{Conditional scores)\}
    \State Init empty $b \times k$ array $C'_t$ \qquad\{Weighted conditional scores, optional\}
    \State Init empty $b \times k$ array $W$ \qquad\{Continuations\}
    \For{$b = 1, \dots, B$}
        \If {$t < L$}
            \State $L[w] \gets \log\pmodel (w | x_{1:t} = X[b])$ \{for all $w \in |V|$\}
        \Else
            \State $L[:] \gets -\infty$
            \State $L[\text{\tt </s>}] \gets 0$ \qquad\{If at the max sequence length, all hypotheses are forced to be complete\}
        \EndIf
        \State $W[b, :] \gets$ words with top $k$ scores in $L$
        \For {$i = 1, \dots, k$}\qquad{}
            \State $w \gets W[b, i]$
            \State $U_t[b, i] \gets S[b] + L[w]$
            \State $C_t[b, i] \gets U[b, :] + \log\pclf(a | x_{t+1} = w, x_{1:t} = X[b])$
            \State $C'_t[b, i] \gets U[b, :] + \alpha\log\pclf(a | x_{t+1} = w, x_{1:t} = X[b])$
        \EndFor
    \EndFor
    \State \{We select new beam elements using $C'_t$, but update $S$ using $U_t$.\}
    \For{$b = 1, \dots, B$}
        \State $b_\text{prev}, i \gets$ $b$-th largest pair of indices into $C'_t$
        \State $S[b,i] \gets U_t[b_\text{prev}, i]$
        \State $X[b] \gets \mathrm{concatenate}\left(X[b_\text{prev}], W[b_\text{prev}, i]\right)$
    \EndFor
\EndWhile
\If {Attribute is deterministic}
    \State $b_\text{best} = 1$
\Else
    \State $b_\text{best} \gets \argmax\limits_{i} C_t[i]$\qquad\{If the classifier is uncertain about the value of the attribute even for a complete output, we take that into account when selecting the output.\}
\EndIf
\State \textbf{Return} $X[b_\text{best}]$
\end{algorithmic}
\end{algorithm}

\section{Related work on conditional generation}
\begin{comment}
Goals: 
- Cover variants CCLM vs attribute
- Describe top-k issue
- Describe why we need to manually work this out instead of just saying "FUDGE but beam search"
- Describe the distinction from VGBS
\end{comment}
The main goal of this chapter is to start bridging the gap between exact search for conditional modes (tractable, but not efficient), and methods that are actually efficient enough to run in practice.
In the last section, we started with ordinary beam search, and derived a version of it that can be used to instead search for conditional modes.

Our goal is to do approximate search on a conditional version of an LM or MT models' unconditional distribution, $\pmodel(x)$.
Because of that, we'll focus on two sampling methods that can be seen as approximately sampling from such a conditional distribution (FUDGE in particular explicitly tries to do so).
We discussed other controllable generations that aren't concerned with conditional distributions in Section~\ref{sec:relatedwork_generation}

\subsection{Two ways to estimate $\pmodel\left(a | x\right)$}\label{sec:modesbeam_alternatives}
 Here we'll look at two approaches to estimating $\prob(a | x_{1:t})$ from partial hypotheses, the methods that introduced them, and the tradeoffs they make.
\paragraph{FUDGE~\citep{fudge}.} FUDGE is a method for conditional sampling, specifically approximately sampling from $\pmodel(x | A(x) = a)$. They train classifiers to predict $\pmodel(a | \cdot)$ conditional on partial hypotheses, just like we need for Equation~\ref{eq:beam_final}.
They apply them to conditional sampling rhyming couplet generation, topic constrained generation, and formality constrained machine translation.

Their approach (and ours) requires calculating $\pclf(A(x) = a \given x_t, x_{<t})$ $x_t$ as an \emph{input} to the classifier.
The problem is that we need to do this for \emph{every} possible continuation token, so the attribute classifier needs to be very lightweight.
On top of that, both FUDGE and our method only apply the classifier to the top $k$ possible next tokens, in order to further reduce compute.

An alternative would be for the classifier to take as input just $x_{<t}$, and then output a $|V| \times |\mathcal{A}|$ matrix that simultaneously predicts the $|V|$ categorical distributions $\pmodel(A(x) = a | x_t, x_{<t})$ (one for each value of $x_{t}$).
This would allow us to avoid the ``top-$k$'' restriction, but would also reduce the capacity of the classifier since it would do computation per possible continuation.

\paragraph{GeDi~\citep{krause2020gedi}.} GeDi (Generative-Discriminators) instead trains class-conditional LMs (CC-LMs) to predict $\prob(x_t | A(x) = a)$ directly.
To use them to modify sampling from an unconditional LM, they use Bayes' rule to estimate $\prob(A(x) = a | x_{1:t})$, which is then applied in the same way as shown in Equation~\ref{eq:bayes}.
In their experiments they train their CC-LMs on labeled datasets rather than model outputs, but to estimate $\pmodel(x_t | A(x) = a)$ you could just train them on model outputs instead.

The upside of GeDi compared to directly predicting $\pmodel(A(x) = a | x)$ is that they don't need to restrict their attribute prediction to the $k$ tokens with the highest marginal scores.
The downside is that training CC-LMs should intuitively be much harder than training classifiers, since they need to learn the entire text distribution.

Imagine training a trivial attribute that was just ``Is the first word of the output 'The'.''
An attribute classifier would only need to predict the marginal probability of seeing ``The'' at the first token, then output either 0 or 1 on all future timesteps depending on what token was output.
A CC-LM would instead try to learn the conditional distribution of all the text following the first token, which is both difficult and completely irrelevant to the classification task.

\begin{table}[h]
    \centering
    \caption{Tradeoffs between the two alternatives discussed for conditional generation (generation from $\pmodel(x | A(x) = x)$).}\label{tab:clf_tradeoffs}
    \begin{tabular}{p{0.1\textwidth}lp{0.2\textwidth}p{0.3\textwidth}}
        \toprule
        Auxiliary model & Predicts & Pros & Cons\\
        \midrule
        Classifier & $\pmodel(A(x) = a | x_t, x_{<t})$ & Doesn't need to learn extraneous information. & Expensive to apply to possible continuations, so only $k$ continuations are considered.\\
        Class-Conditional LM & $\pmodel(x_t \given A(x) = a, x_{<t})$ & Can consider all possible continuations. & Needs to learn next-token distribution in addition to discriminative information.\\
    \bottomrule
    \end{tabular}
\end{table}
\paragraph{Evaluation of tradeoffs} Table~\ref{tab:clf_tradeoffs} summarizes the pros and cons of the two methods.
We chose to use the classifier-based approach since the downside of needing to learn the distribution of text in addition to discriminitave information seemed too large.
That's just an intuitive justification, not an empirical fact, so using conditional beam search with CC-LMs should be tested in future work.

\subsection{Value guided beam search}
Another method for controllable generation which doesn't attempt to do \emph{conditional} generation is Value-Guided Beam Search (VGBS, \citealp{vgbs}).
Our score function in Equation~\ref{eq:beam_final}, is extremely similar in form to the score function used by VGBS.
Specifically, they use:
\begin{equation*}
    S_v(x_{1:t}) = (1 - \alpha) S(x_{1:t}) + \alpha V(x_{1:t})
\end{equation*}
Where $V(x_{1:t})$ predicts the value of a continuation (BLEU score in their experiments).

The differences between VGBS and conditional beam search are due to a difference in goals: Our goal is to find sequences which our LM assigns a high conditional probability to, whereas VGBS is just interested in finding the highest reward sequence.
This difference causes us to select the final best hypothesis differently, and train classifiers differently.

Since VGBS wants to find a high value sequence, they include the weight $\alpha$ in the final score which is used to choose what sequence to output.
They also train their value function on data produced using beam search, since since the ideal value network will be one which can guide beam search specifically to a high scoring output.

On the other hand, we want to actually estimate the quantity $\pmodel (x | A(x) = x)$.
This leads us to use model samples in training, otherwise the classifier will not be trying to predict the conditional under $\pmodel$.
It also means that we take the output from the final beam which is the highest probability under that conditional distribution.
Because of that, when we do use a weight $\alpha$ we only use it during search, and not for final hypothesis selection.

The other difference is that in conditional beam search we may evict a complete sequence which was already found.
This isn't very relevant in standard beam search, since log-likelihoods only decrease as generation continues.
However, using an attribute classifier, it can be the case that the estimate of $\pmodel (a | x_{1:t})$ changes dramatically as a sequence is produced.
A better method would be to keep \emph{all} complete sequences encountered during search, but this isn't usually done, and we leave testing it to future work.\footnote{For regular beam search this would lead to the output being empty whenever the empty sequence is the modal output. This is because the probability of all possible first tokens is calculated, including the EOS token. So ordinary beam search often ``finds'' the global mode, but just doesn't keep track of it and loses it again! This is a manifestation of \citet{meister2020ifbeamsearch}'s point that beam search is probably doing something other than actually trying to find high likelihood sequences.}

\section{Experiments: Length controlled generation}\label{sec:modesbeam_length}
In this section and the next we discuss our experiments with conditional beam search.
Our first experiments are on length-constrained generation for language modeling and MT.
Specifically, our goal is to generate a sequence of exactly length $L$ that has a high score under the relevant model.

Our experiments verify that our method is able to decode outputs of a given length with higher likelihood than those found by beam search.
This shows that conditional beam search can find high-probability sequences which satisfy a constraint.
We also find that, qualitatively, the sequences found using conditional beam search are better than the ones found by just constraining beam search to output at the target length.

\subsection{Models and data}
Our NLG models are the same ones used to find length-conditional exact modes in Chapter~\ref{chapter:modes_exact}: The MarianMT Chinese-English model for MT, and the ROC stories finetuned GPT-2 model for LM.
We train our classifiers using sequences sampled from these models.
In the case of the GPT-2 model we can do this in a data free way (simply generating each text from scratch), but for the MarianMT model we sample translations from the model conditional on sources from the \texttt{news-commentary-v12-zh-en} training data~\citep{wmt17}.

\subsection{Conditioning target: Length}
Because the number of possible output lengths is very high, we train a classifier to predict the length remaining rather than the absolute length of a sequence.
We also reduce the number of categories in the classification problem by bucketing the lengths into coarser groups as the length increases.
Specifically, lengths 0-16 each have a unique class, lengths 17-32 are split into 4 groups, lengths 32-64 are split into two groups, then all lengths 65 and higher are assigned to a single group (24 classes in total).

\subsection{Classifier architecture and training}
For both models, we train a classifier that takes the decoder's hidden states as input.\footnote{The decoder in the case of the LM is the entire model, while the MT model has a separate encoder and decoder.}
This section describes the exact architecture, and how to use it for conditional beam search.
The specific hyperparameters used are given in Appendix~\ref{chapter:beam_hparams_appendix}.

The tricky thing about the classifier is that we want it to be able to make predictions about the class of possible continuation tokens, while not needing to run the full decoder model on each of those continuations to make a hidden state.
To make that possible, the classifier uses the model hidden states at time $t$ (and earlier) to make a classification prediction for time $t + 1$.

We'll formalize the prediction process here.
Let $\bm{h}_{1:T}^{(\ell)}$ be the layer $\ell$ hidden states of the decoder, with the decoder having $M$ total layers and an embedding dimension of $d_\text{model}$.
Suppose we want to predict the final label for an output sequence with a prefix of $x_{1:t}$, and a candidate next token $x_{t+1}$.
In order to make the computation for each continuation lightweight, we frame it in terms of the word embedding of that token\footnote{These embeddings come from the input embedding table from the underlying decoder model.}, $w$.
For some dimension sizes $d_\text{clf}$ and $d_\text{out}$, the classifier output is computed as follows:
\begin{alignat*}{2}
    \bm{h}_{1:t}^{(\text{stacked})} &= \mathrm{Concat} \left([\bm{h}_{1:t}^{(0)}; \bm{h}_{1:t}^{(1)}; \dots; \bm{h}_{1:t}^{(M)}]\right) \qquad && \text{// Concatenate all hidden states layerwise}\\
    \bm{h}_{1:t}^{(\text{in})} &= \mathrm{Linear}\left(\bm{h}_{1:t}^{(\text{stacked})}\right) && \text{// Project down to input dimension: $\mathbb{R}^{T \times (M d_\text{model})} \to \mathbb{R}^{t \times d_\text{clf}}$}\\
    \bm{h}_{1:t}^{(\text{out})} &= \mathrm{Transformer}(\bm{h}_{1:t}^{(\text{in})}) && \text{// $\mathbb{R}^{t \times d_\text{clf}} \to \mathbb{R}^{t \times d_\text{out}}$}\\
    \bm{c}_{t+1} &= \mathrm{Concat}([
            h_t^{(\text{out})},
            w
    ]) && \text{// Concatenate output for time $t$ to token emb.}\\
    \mathrm{Logits}_t &= \mathrm{MLP}(\bm{c}_{t+1}) && \text{// Apply MLP without output dimension $|\mathcal{A}|$}
\end{alignat*}
At training time, the classifier is only passed the tokens that actually occur in the training example, so this is done in parallel for every position in the sequence.
At inference time, it needs to evaluate $k$ candidate continuation tokens (See Algorithm~\ref{alg:beam_cond}).
Since the the transformer output from time $t$ is shared across all evaluations of tokens for time $t+1$, it only needs to be run once for each position, while the MLP is run $k$ times.\footnote{To avoid possible confusion, there are two transformers: the one in the underlying NLG model, and the one being used for classification. Both of them only need to make one forward pass per sequence during training, and one forward pass per token during inference.}

The reason to include the transformer instead of just the MLP is that it allows the classifier to use as many of the NLG model's hidden states as possible, instead of just the hidden states from time $t$.
This is similar to the architecture used by FUDGE, but using a transformer instead of a LSTM.

\subsection{Beam search details}
We use beam sizes of 5 and 20 for our experiments, and always evaluate $k=100$ candidate next tokens for conditional beam search.
We use $\alpha = 1$ as defined in Algorithm~\ref{alg:beam_cond}, so this is exactly the theoretical version of conditional beam search derived in Section~\ref{sec:modesbeam_beam}.


\subsection{Results}\label{sec:modesbeam_length_results}
\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/modes/marian_guided_better_beam=5.pdf}
        \caption{Beam size 5.}\label{fig:marian_beam5}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/modes/marian_guided_better_beam=20.pdf}
        \caption{Beam size 20.}\label{fig:marian_beam20}
    \end{subfigure}
    \caption{A comparison of classifier-guided conditional beam search and beam search when generating outputs that must be a certain length, using the MarianMT Zh-En translation model on the WMT17 dev. set. Each bar shows how often each method finds the higher log-probability output for a given length constraint. The length constraints are relative to the reference sentence, so for a 20 token reference constraints of 16, 18, 20, 22, and 24 tokens were used.}\label{fig:marian_beam_scores}
\end{figure}
    
\begin{figure}    
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/modes/roc_stories_guided_better_beam=5.pdf}
        \caption{Beam size 5.}\label{fig:roc_beam5}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/modes/roc_stories_guided_better_beam=20.pdf}
        \caption{Beam size 20.}\label{fig:roc_beam20}
    \end{subfigure}
    
    \caption{A comparison of classifier-guided conditional beam search and beam search when generating outputs that must be a certain length, using our finetuned GPT-2-345M model on the ROC Stories dev. set. See Figure~\ref{fig:marian_beam_scores} for explanation.}
    \label{fig:roc_beam_scores}
\end{figure}

Our main finding from our length-control experiments is that conditional beam search typically manages to find higher probability outputs of a given length than beam search does.
In these experiments, both beam search and conditional beam search are constrained to output the EOS token at the target length, and never produce the EOS token prior to that point.
We do this by setting the probability of the EOS token to 0 and renormalizing the log-probabilities.\footnote{An alternative would be to just take the top-k tokens that aren't EOS, which would lead to different scores being accumulated across timesteps and could affect the final output. We opted to use the renormalization method since we know that $\pmodel(x_i = \mathtt{</s>} | |x| = L) = 0$ when $i < L$.}

Figures~\ref{fig:marian_beam_scores} and \ref{fig:roc_beam_scores} summarize our findings when controlling the output length.
These plots show how often each method finds the higher likelihood output for a given input and a target length that is rounded from a multiple of the corresponding reference length.
For MT, the source/reference pairs come from the WMT17 dev set.
For the ROC Stories LM, the inputs are the first four sentences of examples from the dev set, and the references are the correct fifth sentence.

Overall, conditional beam search outperforms unconditional beam search in terms of finding high-likelihood sequences satisfying the length constraint.
The closest unconditional beam search comes to being better is at a length ratio of 1.2 on ROC Stories with a beam size of 20, where conditional beam search only finds the better output about 1 percentage point as often.
Unsurprisingly, there is less of a gap between unconditional and conditional search with a beam size of 20.\footnote{If the beam size is increased sufficiently, both methods will eventually find the conditional mode of length $L$.}

One interesting difference between the MT results (Figure~\ref{fig:marian_beam_scores}) and LM results (Figure~\ref{fig:roc_beam_scores}) is that the relationship between improvement and length is inverted.
For a beam size of 5, unconditional search beats conditional search more often at higher lengths for MT, but less often at higher lengths for ROC stories.
A priori we might have expected a trend more like the one shown in Figure~\ref{fig:marian_beam20}, where the benefit of conditional search is the lowest at exactly the reference length, but higher for ``weirder'' lengths which aren't equal to the reference.

\subsubsection{Qualitative properties of outputs}
\begin{CJK*}{UTF8}{gbsn}
\begin{table}[h]
    \centering
    \caption{Selected decoding outputs from MarianMT Zh-En to compare conditional and unconditional beam search (beam size 5). Conditional beam search more consistently leads to grammatical outputs.}\label{tab:marian_beams_selected}
    \begin{tabular}{llp{0.6\textwidth}}
         Type & $\log P(y | x)$ & Text\\
         \toprule
         \input{modes/marian_beam_selected}
    \end{tabular}
\end{table}
\end{CJK*}
\begin{table}[h]
    \centering
    \caption{Selected decoding outputs from ROC stories finetuned GPT2-345M to compare conditional and unconditional beam search (beam size 5). Conditional beam search more consistently leads to grammatical outputs.}\label{tab:roc_beams_selected}
    \begin{tabular}{llp{0.6\textwidth}}
         Type & $\log P(y | x)$ & Text\\
         \toprule
         \input{modes/roc_stories_beam_sequences_selected}
    \end{tabular}
\end{table}
A consistent pattern in the outputs is that conditional beam search finds grammatical outputs of the requested length, while unconditional beam search does not.
Tables~\ref{tab:marian_beams_selected} and \ref{tab:roc_beams_selected} show several examples of this issue.\footnote{To avoid cherry-picking, many more randomly selected outputs are shown in Tables~\ref{tab:marian_beam_samples} and \ref{tab:roc_beam_samples}, that also consistently show the same pattern.}
While conditional beam search finds different outputs for each length such that the final length is correct, unconditional beam search often outputs truncated sequences.

The reason that unconditional beam search is failing is that it can't plan ahead.
If the target length is $L$, ordinary beam search might have no examples on the beam at step $L-2$ that could lead to a fluent ending within two tokens.
The generation models do ``know'' that it's the wrong time to output EOS, so they assign a low-probability to the overall sequence, but that isn't sufficient to find a good output if there aren't any good partial hypotheses on the beam.
This also partially explains why conditional beam search is able to find higher scoring sequences than unconditional beam search.

\section{Experiments: Control of completeness and relevance with LLaMA}\label{sec:modesbeam_llama}
In the last section, we looked at training classifiers to control output length.
This at least directly address the empty-mode problem, but is not of much practical interest.
However, as we saw in Chapter~\ref{chapter:modes_exact}, the 7B parameter LLaMA~\citet{llama} and its derivatives\footnote{No pun intended.} suffer from problems other than brevity.
Some of the problems that exact modes of LLaMA-7B on the instruction-following data displayed were:
\begin{enumerate}
    \item The mode was empty 70.7\% of the time;
    \item Many outputs exactly repeated the prompt;
    \item When the empty output was blocked, the next most likely output was often a \LaTeX fragment;
\end{enumerate}
However, when the output distribution has low enough entropy, the modal output was sometimes a response to the prompt.
The question we investigate in this section is whether we can condition away these problems and get high-quality responses from LLaMA-7B despite it not having been trained for anything other than pure language modeling.

We define two attributes to use for conditioning: ``Completeness'' and ``Irrelevance'', defined fully in Section~\ref{sec:modesbeam_attributes}.
We want outputs with high completeness, but low irrelevance.
With only 200 labeled training examples for each of these categories, we are able to steer LLaMA-7B to produce beam search outputs that display the problems above much less frequently.
This is extremely promising for our goal of improving generation without needing to destroy the information stored in the underlying language model.

\subsection{Model and data}
These experiments use the LLaMA-7B model, which has only been trained for language modeling, not instruction following.
We chose to use this over the finetuned models such as Alpaca~\citep{alpaca}, since those models have been directly trained to respond to prompts, while we're interested in trying to get high-quality behavior out of a generic LM.
Rather than using LLaMA in its 16-bit precision, we use a 4-bit quantized version (See Section~\ref{sec:modesbeam_llama_clf} for details).

We used 500 inputs from the Alpaca~\cite{alpaca} as inputs for classifier training.
For each input, we generated a completion using the ``beam search'' prompt format shown in Appendix~\ref{chapter:prompts_appendix}.
450 of these are used for training the classifiers, and 50 are used as a validation set for early stopping.
These completions were generated using beam search, instead of sampling.
We discuss the reason for making that choice in Section~\ref{sec:modesbeam_concessions}.

For testing, we use inputs from the \texttt{databricks-dolly-15k} dataset~\citep{dolly15k}.
We switch datasets for evaluation to make it less likely that any improvements we see are just due to the classifier exploiting idiosyncracies of the training data.
In order to make our output length limit not too constrictive, we use the 248 prompts from the dataset which led to a prompt length of under 100 tokens.

\subsection{Conditioning targets: Completeness and Irrelevance}\label{sec:modesbeam_attributes}
We train two separate classifiers for the following two attributes:
\begin{itemize}
    \item Completeness: The degree to which an output attempts to fully answer the prompt. For the question ``Who was the first president of the United States?'', ``Abraham Lincoln'' would be a complete answer despite being incorrect. ``I don't know'' would be incomplete, as would an empty output.
    \item Irrelevance: The amount of unnecessary text in the output. An empty output has minimal irrelevance by definition, while ``\textbackslash{}text\{George Washington\}'' would be somewhat irrelevant due to the unnecessary TeX markup.
\end{itemize}
By controlling for both of these attributes at the same time, we are implicitly assuming that the events ``$x$ is complete'' and ``$x$ is relevant'' are independent conditional on a prefix of $x$.
That is definitely untrue, so this is an approximation.

For training data, we labeled 500 outputs from LLaMA-7B for completeness, while the GPT-4 was used to predict the irrelevance. (See Appendix~\ref{chapter:prompts_appendix} for the exact prompt used).
The labeling was done on a scale of 1-5, but the final classification task was binary classification.
All empty outputs were automatically marked as a 1 for Completeness, and a 1 for Irrelevance.
The class balances were:
\begin{itemize}
    \item Completeness: 70\% incomplete, 30\% complete;
    \item Irrelevance: 13.8\% irrelevant, 86.2\% relevant;
\end{itemize}
See Section~\ref{sec:modesbeam_concessions} for discussion of concessions we had to make in terms of training data quality.

\subsection{Classifier architectures}\label{sec:modesbeam_llama_clf}
The classifiers we use in this section consist of taking the LLaMA-7B model, adding a linear classifier on top of its final layer hidden state, and partially finetuning the model.
The reason for using this much more heavyweight approach than in the last section is that we only have 500 labeled training examples, so leveraging the pretrained information available in LLaMA\footnote{Both about the distribution of text and the meaning of its hidden states.} is critical.

However, if we made classifiers exactly as stated above, the memory for the parameters alone would take:
\begin{equation*}
(7\text{ billion}) \times (16\text{ bits}) \times (3\text{ models}) \approx 42 \text{ GB}
\end{equation*}
We ran these experiments on a single 24 GB GPU, and the total above doesn't even include the model activations, so we use several methods to reduce the footprint.

Our method is based on QLoRA~\citep{qlora}, a parameter-efficient fine-tuning method for large models consisting of the use of 4-bit blockwise quantization, and LoRA~\citep{lora}.
We'll briefly go over each of those methods here as background, then discuss what modifications we made.
For specific hyperparamters, see Appendix~\ref{chapter:beam_hparams_appendix}.

\paragraph{4-bit blockwise quantization.} We use the blockwise quantization method introduced by \citet{qlora}, but with the AF4-64 code\footnote{See: \url{https://github.com/davisyoshida/abnormal-floats}.} instead of their NF4 code.
Blockwise quantization of a transformer replaces each floating point weight matrix with a matrix of integers, although with a scaling value per block (in our case each block consists of 64 values).
When the weight is needed for a quantization, the values are turned back into 16-bit floating point values by taking the relevant value in the quantization code, and multiplying it by the scaling value for the block.
In the case of LLaMA-7B, this reduces the GPU memory needed to store the weights from 13.5 GB to 3.7 GB.

\paragraph{LoRA \citep{lora}.} Low-rank Adaptation (LoRA) is a method for finetuning a large model without needing to update its weights, and in particular without needing to maintain optimizer states for those weights.
For each weight matrix $W \in\mathbb{R}^{m \times n}$ to be trained, new weights $A \in \mathbb{R}^{r \times n}$ and $B \in \mathbb{R}^{m \times r}$ are introduced.
Then, each multiplication $Wx$ in the network is replaced by the computation $Wx + BAx$.
$B$ is initialized to be the zero matrix, so this initially makes no difference to the model's output.
The combined set of $A$'s and $B$'s for the whole model is often also referred to as a LoRA.\footnote{Presumably short for low-rank \emph{adapter} instead of \emph{adaptation} in this case.}

Instead of training $W$, it is left frozen and $A$ and $B$ are trained instead.
Since $r \ll \min (m, n)$, this leads to far fewer parameters being trained, and is equivalent to learning a rank $r$ update.
Readers should see \citet{lora} for more information.

\paragraph{Batching LoRAs.} With limited GPU memory, the idea of loading more than one 7 billion parameter model into memory sounds too expensive to be practical. However, if each one of those models is just a LoRA finetune of the same underlying base model, we can load a single copy of the quantized base-model, and the much smaller LoRA parameters for each finetuning.
On top of the memory savings, we can vectorize forward passes by batching the $A$ and $B$ matrices from each LoRA together.
In our case we'll have three LoRAs: One for each of the two classifiers, and an additional one that has $A = B = \bm{0}$ to retain the behavior of the original LM\footnote{This is inefficient since computing $ABx$ for the zeroed out parameters is a waste of computation, but it lets us simplify the implementation.}.
So, for each ``model'' a matmul that originally mapped from $\mathbb{R}^{m}$ to $\mathbb{R}^{n}$ is batched to map from $\mathbb{R}^{3 \times m}$ to $\mathbb{R}^{3 \times n}$.

This is implemented without any changes to the model code, since we use a custom JAX~\citep{jax} transform for applying LoRA to models that were written without LoRA in mind\footnote{The transformation is available at \url{https://github.com/davisyoshida/lorax/tree/master/lorax}, and should be compatible with most JAX models.}.
We then use JAX's \texttt{vmap} transformation to turn a function that expects a single LoRA into one that takes multiple LoRAs and produces multiple outputs from a single input.

\paragraph{Shared trunk.} This would still use way too much memory, since we'd still need to store three full copies of the KV-cache during inference. 
For beam search, this is also multiplied by the beam size, which would make running decoding on a single GPU impractical.
We reduce this amount by only training LoRA parameters on the last three of LLaMA's 32 layers.
This way, the LoRA finetuned classifiers can still take advantage of LLaMA's pretrained knowledge to some extent, but they only need distinct key-value caches for the final few layers.

The final outcome of this is that we only need to store a cache that is about $(29 + 3 \cdot 3)/32 \approx 1.19$ times the size that would be needed for just the LM alone.
We chose to do this instead of the transformer method used for length prediction in order to significantly increase the capacity of the classifiers, as well as letting them make better use of LLaMA's pretraining in order to learn from just 500 examples.

\paragraph{Lookahead batching.} Recall that Algorithm~\ref{alg:beam_cond} requires applying the classifier to $k$ candidate continuations for each of the $B$ beam hypotheses.
The trick to doing this efficiently is to batch over the candidates, but have all candidates share a single key-value cache.\footnote{This works since all candidates for a given hypothesis on the beam share a history. If we're looking at candidate outputs for position $t+1$, all hidden states up until $t$ will be identical.}

For this type of batching, we do need to modify the model code as well.
The reason is that naive batching would also lead to a batched output of the updated key-value cache, i.e., $B \times k$ copies of it.
To avoid that, we modify the LLaMA code to instead only output the key and value vectors for the $t$-th timestep.\footnote{This also requires modification of the attention mechanism. All reductions that go from time $1$ to $t$ are modified to handle timesteps $1$ to $t-1$ in a group, then the result for the present timestep is handled separately.}
After we select which tokens will be used for the next timestep, we make a single updated cache for each beam element, so that we never need to instantiate more $B$ key-value caches.

\paragraph{Summary of modifications to LLaMA.} The original LLaMA model is a function that has the following inputs:
\begin{enumerate}
    \item Model parameters
    \item Key-value cache
    \item Input token (At inference time just a single token would be input)
\end{enumerate}
and outputs:
\begin{enumerate}
    \item Classification or Next-token prediction logits
    \item New key-value pairs
\end{enumerate}
We modify it into a function that has the following inputs:
\begin{enumerate}
    \item Model parameters
    \item LoRA parameters (Batch axis: \texttt{lora})
    \item Key-value caches for each beam element and group of LoRA parameters (Batch axes: \texttt{lora} and \texttt{beam})
    \item One token for each of $k$ continuations of each beam element (Batch axes: \texttt{beam} and \texttt{continuation})
\end{enumerate}
and outputs:
\begin{enumerate}
    \item Classification \emph{and} next-token logits (Batch axes: \texttt{lora}, \texttt{beam}, \texttt{continuation})
    \item New key and value \emph{vectors} for the most recent timestep, which can be used to update the caches (Batch axes: \texttt{lora}, \texttt{beam}, \texttt{continuation})
\end{enumerate}
Note that for the key and value vectors, the \texttt{lora} batch axis is only present for the last three layers, since those are the layers we finetune.

\subsection{Beam search details}
We use a beam size of 5 for all experiments in this section.
To reduce the cost of training and inference, we limit the max sequence length to 196 tokens (including the prompt).
We evaluate $k=100$ candidates for conditional beam search, and use a weight of $\alpha = 2$.


\subsection{Weaknesses in classifier training}\label{sec:modesbeam_concessions}
Unlike in our length control experiments, we have to make various compromises in classifier training just due to resource constraints.
All the changes here should make the classifier \emph{worse} so we expect an implementation of conditional beam search without these limitations would have \emph{better} final performance.

\paragraph{Labeling budget.} The main constraint is that we have an extremely limited data labeling budget (both in terms of time and money), so we only use 500 training examples for each classifier.
Contrast this with the hundreds of thousands of training examples we were able to use for the length control classifier.

\paragraph{Unrepresentative training data.} Related to the above point, we had to generate the training data using beam search on LLaMA, rather than sampling.
The issue is that there are two things we need for training data to be effective for training an attribute classifier.
The first is that it should be representative of the model's output distribution, $\dmodel$.
The second is that the data should be representative of the types of inputs that the classifier will be used on at inference time.

These are conflicting goals, which we can explain with an example.
Consider the prompt ``Name three scifi/fantasy book series.''
Imagine that the beam search completion is ``1. Harry Potter, 2. Lord of the Rings, 3. Foundation.'', and a sample output is ``Some popular series are: Mistborn, The Expanse, and The Three Body Problem series.'' We want the classifier to be able to handle prefixes of the beam search output as input, but its predictions are \emph{about} the sampling output, which has different properties than the beam search output.

Due to our limited budget, we optimize for input validity over output validity, and use beam search completions from LLaMA-7B as our training data.
The ideal solution would be to use a wide enough range of samples that they achieve good coverage of model behavior, or to use outputs that start by using beam search but sample completions.\footnote{This latter strategy is the opposite of what VGBS does: \citet{vgbs} sample the start of the model decoding and complete it using beam search.}

For context on the difference in scales, the recently released LLAMA-2 Chat model was trained using over 1.4 \emph{million} human preference labels\citep{llama2}.
Using that scale of human labeling, we wouldn't need to make this compromise in terms of our data distribution.

\subsection{Results}
We find that, despite the weaknesses in classifier training discussed in the previous section, we're able to generate much more acceptable results from LLaMA-7B using conditional beam search than ordinary beam search.

\subsubsection{Classifier satisfaction}
\begin{table}[h]
\centering
\caption{Effect of conditioning on LLaMA-7B beam search outputs. ``\% of outputs'' is the percent of outputs for which the classifier predicted the attribute was the majority class. $\prob_\text{clf}(a)$ is the average of the classifiers predicted probability over the outputs.
The outputs in the conditional row are the same for both classifiers (i.e., both classifiers were used simultaneously to guide generation).}\label{tab:classifier_satisfaction}
\begin{tabular}{llllll}
  & Method & \multicolumn{2}{c}{Completeness $(\uparrow)$}  & \multicolumn{2}{c}{Irrelevance $(\downarrow)$} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6}
  &                    & \% of outputs & $\prob_\text{clf}(a)$ & \% of outputs & $\prob_\text{clf}(a)$ \\ \midrule
 & Beam search             & 92.34             &  0.5999 & 45.56     &  0.4996\\
  & Conditional beam search & \textbf{98.39}    & \textbf{0.6289} & \textbf{27.02}    & \textbf{0.3583}\\ \bottomrule 
\end{tabular}
\end{table}
The easiest measurement we can do is to look at how often the attribute classifiers label complete outputs as having satisfied the target.\footnote{We didn't do this in the previous section since we could directly constrain the outputs to be the right length. The classifier satisfaction would have been 100\% in all cases (or whatever the highest value it could output is).}
Table~\ref{tab:classifier_satisfaction} shows the classifier prediction statistics for the unconditional and conditional LLaMA-7B outputs.
For both completeness and irrelevance, using conditional beam search satisfies the classifier more often.

One thing to point out is that the classifier seems to predict that outputs are complete far more often than they actually are.\footnote{This can be verified by looking back at the statistics about degenerate outputs from the start of the chapter.}
Even though it isn't good in absolute terms, the classifier is still effective in terms of guiding beam search, as we'll see in the next few sections.

\subsubsection{Improvement in identified degeneracies}
\begin{table}[h]
    \centering
    \caption{Improvement in occurrence of degenerate outputs from using conditional beam search with LLaMA-7B. These were measured using 248 prompts from the \texttt{databricks-dolly-15k} dataset.}\label{tab:beam_heuristics}
    \begin{tabular}{lll}
        Behavior & Beam search & Conditional beam search\\
        \midrule
        Empty output & 18.6\% & 0.0\%\\
        Spurious TeX & 6.5\% & 0.0\%\\
        Repeating prompt & 29.0\% & 4.8\%\\
        \bottomrule
    \end{tabular}
\end{table}
 At the start of this chapter, we mentioned several problems we observed, namely: empty outputs, repetition of the prompt, and emission of unecessary TeX code.
These problems were dramatically improved by the addition of conditioning.

Table~\ref{tab:beam_heuristics} shows the frequency of each problem under each type of beam search.\footnote{Even though LLaMA's exact mode is empty about 70\% of the time, beam search doesn't usually find that out.} The rate of these three undesired behaviors drops significantly when attempting to condition on Completeness and Relevance.
The classifier seems to be learning non-trivial behavior, not just lexical rules.
For example, given the input ``Output a LaTeX table'', it still TODO.

\subsection{Qualitative analysis}
We'll now look at some examples of interesting behavior that the conditional beam search outputs show.
Appendix~\ref{chapter:beam_appendix} shows the outputs with and without conditioning for a non-cherrypicked subset of the Dolly-15k prompts.

\subsubsection{Responses to factual but high-entropy prompts}
As we saw in Chapter~\ref{chapter:modes_exact}, inputs with a high-number of possible responses are more likely to have the empty sequence as their mode.
While we wouldn't recommend using MAP for something like poetry generation, it's easy to come up with prompts that are requesting concrete factual information, but also have a large number of possible responses.
Here's an example:
\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \textbf{Prompt:} ``Suggest three restaurants in Chicago.''\\
    \textbf{Beam search:} \texttt{<empty>}\\
    \textbf{Cond. beam search:} ``1. Lou Malnati's\\
    2. Giordano's\\
    3. Gino's East''
\end{mdframed}
Here, any three restaurants will do, but there are many possible responses, so it's unsurprising that unconditional beam search gives an empty response.

Here's another example where there are many ways to choose to answer, but once a choice is made there's no ``creativity'' required:
Here's an example:
\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \textbf{Prompt:} ``Translate the phrase "PhD thesis" into 5 languages''\\
    \textbf{Beam search:} \texttt{<empty>}\\
    \textbf{Cond. beam search:} ``* French: thèse de doctorat\\
* German: Dissertation\\
* Italian: tesi di dottorato\\
* Portuguese: tese de doutorado\\
* Spanish: tesis de doctorado''
\end{mdframed}
The German translation is incorrect, but the conditional beam search output is high-quality, while beam search only finds the empty sequence.

\subsubsection{Factual uncertainty}
There may also be cases where the model is uncertain about the answer, but conditional on the answer the output is highly constrained. This example shows how even factual questions can cause degenerate outputs from the base model:
\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \begin{CJK*}{UTF8}{gbsn}
    \textbf{Prompt:} ``What is the literal and figurative meaning of "雪中送炭"?''\\
    \textbf{Beam search:} ``雪中送炭\\\\雪中送炭\\\texttt{<continues repeating>}''\\
    \textbf{Cond. beam search:} ``The literal meaning of "雪中送炭" is "to send coal in the snow".''
    \end{CJK*}
\end{mdframed}
Conditional beam search only half answered the question, but unconditional beam search ends up in meaningless repetition.\footnote{This particular case wouldn't have been caught by our ``repeating the prompt'' heuristic since the output isn't an exact suffix of the prompt.}

\subsubsection{TeX outputs}
Here are two examples of outputs where the ``TeX problem'' is fixed:
\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \textbf{Prompt:} ``Name three famous AI researchers''\\
    \textbf{Beam search:} ``\textbackslash{}begin\{itemize\}\\
\textbackslash{}item Alan Turing\\
\textbackslash{}item John McCarthy\\
\textbackslash{}item Marvin Minsky\\
\textbackslash{}end{itemize}''\\
    \textbf{Cond. beam search:} ``Alan Turing, John McCarthy, and Marvin Minsky''
\end{mdframed}
In this one, the same response is output, just without the unnecessary markup.

\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \textbf{Prompt:} ``Can you share a response of politely informing the customer that we dont support a feature''\\
    \textbf{Beam search:} ``\textbackslash{}begin\{blockquote\}\texttt{\textbackslash{}n\textbackslash{}n}\textbackslash{}begin\{blockquote\}\texttt{\textbackslash{}n\textbackslash{}n}\texttt{...<repeated>}''\\
    \textbf{Cond. beam search:} Thank you for your inquiry. I am sorry to inform you that we do not support your request at this time.
\end{mdframed}
In this one, beam search collapses to a degenerate output, while conditional beam search finds a bland but correct response.\footnote{ ``Bland but correct'' is basically what we want out of a good MAP-style algorithm. See Section~\ref{sec:modestheory_templates} for discussion of why this is expected.}

\subsection{Discussion: Conditional beam search with LLaMA}
Despite only using a tiny amount of labeled data, we were able to guide LLaMA-7B to produce better outptuts using conditional beam search.
In particular, the rates of each of the three degeneracies we targeted decreased significantly.
Qualitatively, we see that we are able to find outputs of reasonable quality using conditional beam search.
This is true even for inputs with high output entropy, which ordinary beam search will tend to produce trivial responses to.

However, there are still problems present in the outputs of conditional beam search.
At least some of these are likely due to the classifier being too weak.
As shown in Table~\ref{tab:classifier_satisfaction}, the Completeness classifier predicted that 92\% of beam search outputs are complete, which is very much at odds with our measured rates of output degeneracy.
To address this, we will need to train better classifiers, both by using more labeled data, and by improving the training procedure.
A more accurate classifier should lead to even higher quality outputs, allowing us to investigate how far we can go without any tuning of the underlying model.

\subsection{Future work: Performance improvements}\label{sec:modesbeam_perf}
Our main goal in these experiments was to find out what was possible by purely guiding beam search, instead of modifying the model weights themselves.
This led to a method that worked, but was very slow.
Generation from LLaMA-7B with two attribute classifiers, $k=100$ and a beam size of 5 runs at about 1 token/second on an NVIDIA Quadro RTX 6000 GPU, which is far too slow to be practically useful.
In this section we discuss how conditional beam search can be made more efficient.

\paragraph{Custom GPU kernels.} Our experiments use pure JAX implementations of 4-bit dequantization and attention.
Using optimized GPU kernels would significantly improve performance.
See \citet{qlora} for information on 4-bit matmul kernels, and \citet{flashattention2} for an optimized attention implementation.

\paragraph{Varying $k$.} We fixed the value of $k$ (the number of candidate next tokens to consider) to 100 in all our experiments. Because we only need to look at high likelihood tokens, it's possible that a much lower value of $k$ would not change generation outputs. To find the minimal value of $k$ that would leave the outputs unchanged, we could just record the rank of each token selected during decoding (in terms of the original model's likelihood of each token). If the top 5 tokens in conditional likelihood only come from the top 20 tokens in terms of unconditional likelihood, we could get a large speedup.

\paragraph{Classifier architectures.} The reason we used an expensive classifier architecture was so that we could take advantage of LLaMA's pretraining to manipulate its own hidden states.
Using more training data should allow us to train classifiers from scratch with a similar architecture as used in Section~\ref{sec:modesbeam_length}.
Alternatively we could still train the costly LoRA-based classifiers, then use model distillation to create a cheaper classifier.

\subsection{Further Future work}
As we said in Chapter~\ref{chapter:modes_theory}, we see both conditional sampling and conditional search as promising ways of improving output quality.
In this chapter we focused on conditional search, but hope to look at conditional sampling in the future.
Instead of conditioning away the problems of search outputs: emptiness and reptition, we would instead try to condition on things such as fluency and factual correctness, which suffer when sampling.

The main direction for future work on conditional search is to scale up the experiments, both by training on more data, and by testing on larger models.
We discussed implementation efficiency as a particular focus in Section~\ref{sec:modesbeam_perf}.

\section{Conclusion}
In Chapter~\ref{chapter:modes_exact} we found that length-conditional modes for NMT and story completion were often high quality, as opposed to continuing to suffer from the ``bad mode'' problem even after conditioning.

This inspired us to see if we could find a more practical approach to search for conditional modes, which we did in this section.
Our length-constrained generation experiments that used beam search with the conditional distribution, $\pmodel(x | |x| = L)$, successfully allowed us to find higher scoring sequences satisfying the length constraint than those found by beam search.
These sequences tended to be grammatical far more often than those found by ordinary beam search, so in this case the difference in likelihood was reflected by a difference in quality.

We then moved on to the more ambitious goal of improving the instruction-following behavior of LLaMA-7B, a model that was not trained for instruction following.
Using only 500 labeled training examples for ``completeness'' and ``irrelevance'' we trained classifiers with a novel architecture that allowed us to implement conditional beam search.
The outputs were higher quality than ordinary beam search, both in terms of our automated measures of degenerate outputs, and qualitatively.

We aren't claiming that this method is currently ready to replace sampling based methods for NLG, but we see it as a promising step towards more powerful MAP based methods.
Using attribute classifiers to fix output degeneracy lets us get high quality outputs \emph{without} needing to finetune the underlying language model at all, which is the goal we laid out in Chapter~\ref{chapter:modes_theory}.

==> modes/exact_chapter.tex <==
\chapter{Exact Modes in Machine Translation, Story Completion, and Instruction Following}\label{chapter:modes_exact}
\begin{comment}
Things to go over:
- Overall framing:
    - S&B identified that exact modes were bad
    - Had some statistical results of length conditional modes
    - We'll replicate their result
    - Extend it to GPT-2 finetuned on ROC stories
    - Extend it to Alpaca-7B and Guanaco-7B
    - Takeaways:
        - On MT and even ROC stories, there's not really a ``multi-layer'' bad mode issue: Once you condition the length you basically get good outputs
        - On LLaMA derivatives, we do observe other issues: <nooutput> from Alpaca, 
    - We'll qualitatively look at some length conditional modes and see that they're not terrible
    - On llama variants we can look at what properties cause the mode to be empty
- Point about being careful to not use early t
\end{comment}

In the previous chapter we argued that the bad mode problem might be due to properties of our training data distributions, and therefore is not necessarily evidence of model error.
If correct, this implies that no amount of improvement in modeling will overcome the likelihood/quality mismatch.
Because of this, we suggested that one possible decoding method would be to search for the mode of conditional distributions of the (optimistic) form $\prob \left(x \given \text{$x$ is not degenerate}\right)$.

The main question to be answered is: if we condition away one issue, such as empty outputs, will we just run into another degeneracy such as repetition or disfluency?
In this chapter we give some evidence that \emph{conditional} model modes are often high-quality if we condition away the specific problem of length-degeneracy.
However, not only do we find that the problem hasn't abated with scale, we also find that there are several issues with exact modes in a family of larger language models when they are applied to an instruction following task.
These findings come from case studies of exact model modes for three tasks: Machine translation (MT), cloze completion, and open-ended instruction-following/question answering.
The interesting implication is that while many model modes of larger scale models are degenerate in various ways, many are not, suggesting that conditioning away the problems may be a viable path forward.

\paragraph{NMT and Cloze completion.} First, we replicate \cite{catgotyourtongue}'s finding of NMT models having the empty sequence as their mode, and find the same result with a language model trained to complete stories from the ROC stories~\citep{roc_stories} corpus.
However, when we instead search for \emph{length-conditional} modes, we find that they're generally high-quality, rather than just displaying other problems such as repetition.
This suggests that it might not be too hard to condition away the bad types of atypicality discussed in the last chapter.

\paragraph{Scaling up with LLaMA.} We also report, for the first time, on the exact modes of more modern language models, specifically from the LLaMA~\citep{llama} model family.
We find unconditional modes for instruction-following inputs for LLaMA-7B, Alpaca-7B~\citep{alpaca}, and Guanaco-7B~\citep{qlora}, and find:
\begin{itemize}
\item Despite these models having over an order of magnitude more parameters than the previous generation of models, their modes are still often empty.
\item When the mode for the instruction finetuned models is not empty, it is usually high quality.
\item The mode is more likely to be empty when the input is more open-ended. We verify this both qualitatively and quantitatively.
\item LLaMA-7B's modes \emph{do} display degeneracies other than emptiness.
\end{itemize}

Overall, our findings show that all the models we test have fairly high-quality global modes, \emph{except} for certain degeneracies which we discuss.
In the next chapter we will take advantage of this fact to develop a version of beam search that approximately searches for high-scoring sequences while avoiding degenerate outputs.

\section{Background: Exact modes of NLG models}
It's commonly assumed that exact MAP decoding from autoregressive NLG models is intractable due to the exponential size of the search space, but this is not correct.
\citet{catgotyourtongue} pointed out that simple depth-first search (DFS) with pruning can find the exact modal output of NMT models, since the properties of the search problem make it so that aggressive pruning is possible.
For example, \citet{stahlberg2022uncertainty} showed that the exact mode could usually be found for a transformer MT model while searching less than 1 million states.

To show how pruning works, here's a quick example.
Suppose that during tree search, a complete translation with a (model) probability of $1/5000$ has been found.
Two observations are necessary:
\begin{enumerate}
    \item Any partial hypothesis with a probability less than $1/5000$ can be discarded, since adding any more tokens can only lower the probability.
    \item Every search node gives you a possible complete hypothesis to consider, since you'll already be evaluating the probability of every possible continuation, including the next token being EOS. (And complete hypotheses are exactly the sequences that end in EOS).
\end{enumerate}
These features make it possible to prune an enormous fraction of the search space, making exact inference tractable.

As mentioned in the last chapter, this method showed that over half of the source sentences they tested on had the empty sequence as their modal translation, and longer source sentences were \emph{more} likely to have an empty modal translation.

It's already implicit in how we use beam search that we're not \emph{really} looking for high scoring outputs.
If someone wanted to find higher scoring outputs with beam search, they could make (beam size) $\times$ (sequence length) complete hypotheses by just adding EOS to each partial hypothesis considered during search.
This takes no extra model forward-passes, since the probability of every next token (including EOS) is already calculated when new hypotheses are being generated.
This would let ``beam search'' with a beam size of 1 find the empty sequence when it's the modal translation.

We don't want to find these outputs, so we don't make this ``improvement'' to beam search.
\citet{meister2020ifbeamsearch} suggested that beam search may actually be the most successful decoding method because it has a useful inductive bias, which could explain why it is still useful, even if making the beam size larger or considering more hypotheses is harmful.

\citet{stahlberg2022uncertainty} look at search for exact modes in more depth.
They look at the relationship between intrinsic uncertainty (whether an input allows many different outputs), search errors, and how many states DFS explores before finding the mode.
They operationalize intrinsic uncertainty as average edit distance between references divided by average reference length, for multi-reference tasks.
They find that more uncertainty leads to DFS taking longer to find the mode. 
They also find the $N$ highest scoring sequences for each task, and find that those sequences do actually represent a larger fraction of the total probability mass for inputs with lower intrinsic uncertainty (i.e., GEC inputs or shorter MT inputs).

\section{Optimizing memory usage for DFS on transformers}\label{sec:modesexact_dfs_mem}
In this section we'll briefly describe a method for reducing the memory usage necessary for running DFS on transformer NLG models.
Generating from a transformer requires caching the key and value vectors for previous timesteps, in order to avoid a large amount of recomputation for each token.
Running DFS to depth $k$, and storing a KV-cache of length $k$ at each nodes, leads to storage that is quadratic in $k$, even though only $k$ nodes are active at a time.

For the MT and GPT-2 models we experiment with, the maximum search depth and hidden state dimension are both small enough that we can do this with no issue.
The LLaMA-based models however, are over an order of magnitude larger, and also frequently lead to searching subtrees that are hundreds of tokens deep.
As such, we need some way to avoid actually storing a full KV-cache at each node.

Empirically, the DFS search order for these models often involves some path through the search tree being greedily expanded, without any branching.
That is, many search nodes will only have one child which gets explored.
For these nodes, storing the KV-cache for later is a waste of memory since it will never be re-used.
We don't know up-front which nodes will and won't be re-used, but we can still save some memory without losing too much performance by taking a heuristic approach.

To reduce storage while still avoiding running the model on a prefix more than once, each search node initially only stores the hidden state for the token that it used as input.\footnote{Our implementation of DFS is just recursive, so when we say that a search node stores something, we mean that it's stored in the Python interpreter's stack frame for that call to the DFS function.}
Once a node's second child is about to be expanded, the full KV-cache is reconstituted from the keys and values stored at that node and in its ancestors.
Specifically, the node uses back pointers to go back up the search tree until some node that has a full KV-cache is found.
This way, a greedy search path out to depth $k$ will only require $O(k)$ memory instead of $O(k^2)$.

In summary, when search node at depth $k$ is evaluated, a $k \times d$ key/value cache\footnote{The KV-cache is actually a list of a key and value cache for each layer, so the size-$d$ dimension should be seen as a concatenation of all these different values.} $\bm{h}_{1:k}$ is produced
It is then processed as follows:
\begin{enumerate}
    \item The search node saves the vector $\bm{h}_{k}$
    \item The full cache $\bm{h}_{1:k}$ is passed to the first child node, which uses it for a forward pass then frees it
    \item If a second child node will be expanded, the search node recomputes the full cache $\bm{h}_{1:k}$ using its cached vector and those cached in its ancestors. This time the cache is saved for use in the third, fourth, etc. child instead of being freed after the second child uses it.
\end{enumerate}

This heuristic isn't optimal by any means, but it lets us avoid running out of memory when the search state gets hundreds of nodes deep.
Some potentially better methods include using a LRU cache that limits the number of full caches in memory, or using the next-token probabilities at each node to make a smarter decision about whether a full or partial cache should be kept.

\section{Exact modes of an MT model}
In this section, we use DFS to find the exact modes of the pretrained Chinese-English MarianMT model~\citep{marianmt} on the WMT'17 Zh-En \texttt{newsdev} dataset~\citep{wmt17}.
The model is a standard transformer using the architecture of \citet{vaswani2017attention}.
Just like \citet{catgotyourtongue}, we find that the model's mode is often empty, and that this occurs more often as the length of the source sentence increases.
In addition to replicating their results, we also qualitatively examine the modal outputs to see if the the empty modes were just hiding further degeneracies (e.g., disfluency or repetition).

One important thing to note about this model is that it was trained with 10\% label smoothing.
This means that the model is trained with a (token-wise) 90-10 mixture distribution of actual translations and the uniform distribution on its vocabulary.
This mixture distribution puts a hard upper bound on how long the modal output can be (See \citet{liang2022implicit}), but \citet{riley2022continuum} found that adding label smoothing didn't tend to change the length or repetition bias in beam search, so this level of label smoothing might be too small to change the actual modal sequence.

\subsection{Unconditional modes}
\begin{figure}
  \centering
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/marian_frac_empty_vs_srclen.png}
    \caption{Percent of source sentences that have the empty sequence as their modal output.}
    \label{fig:mt_empty_percent}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/marian_empty_prob_src.png}
    \caption{Geometric mean of the model's probability of the empty sequence given the input.}
    \label{fig:mt_empty_prob}
  \end{subfigure}
  \caption{MarianMT Zh-En predictions of empty outputs on WMT17 Zh-En \texttt{newsdev-2017} set (2002 examples). Source sentences are grouped into 10 equally sized bins by length.}
  \label{fig:mt_empty_srclen}
\end{figure}

As expected, we find that the MarianMT Zh-En model predicts that the empty sequence as the mode for 57.7\% of the 2002 source sentences.\footnote{For reference, \citet{catgotyourtongue} found that 51.8\% of inputs on the WMT \texttt{news-test-2015} En-De dataset had an empty mode under their model.}
Figure~\ref{fig:mt_empty_srclen} shows the relationship between the length of the input sentence and empty outputs.
Just like \citet{catgotyourtongue}, we find that longer source sequences are \emph{more} likely to have an empty modal output (Figure~\ref{fig:mt_empty_percent}. 
We can also just read the probability of generating an empty output directly off the decoder logits, which is shown in Figure~\ref{fig:mt_empty_prob}.
It shows that the average log-probability of the empty output only goes from about 1 in 10,000 to 9 in 100,000 as the source length increases.

These results are consistent with the explanation given in Chapter~\ref{chapter:modes_theory}: The main cause of the empty mode problem is that the entropy of valid outputs increases with input length, but the probability of the empty output does not decline fast enough to offset this effect.

\subsection{Length-conditional modes}
\begin{table}[h]
    \begin{CJK*}{UTF8}{gbsn}
    \centering
    \caption{Global and length-conditional modal translations of ``泰国旅游景区炸弹爆炸致四人死亡'' by the MarianMT Zh-En translation model. The reference translation is ``Thailand Bomb Blasts At Tourist Hotspots Kill Four'' (14 tokens).}\label{tab:marian_example}
    \begin{tabular}{lll}
         Length constraint (tokens)&  Log-probability & Text\\
         \midrule
        Global mode & -7.91 & \texttt{</s>} \\
        4 & -9.22 & Four people died\texttt{</s>} \\
        6 & -9.77 & Four people were killed.\texttt{</s>} \\
        8 & -10.37 & In Thailand, four people died.\texttt{</s>} \\
        10 & -10.63 & A bomb blast in Thailand killed four people.\texttt{</s>} \\
        12 & -9.60 & The bombing of the Thai tourist zone killed four people.\texttt{</s>} \\
        \bottomrule
    \end{tabular}
\end{CJK*}
\end{table}
We'll now look at \emph{conditional}-modes of this model, which are the exact values of:
\begin{equation*}
   y^* = \argmax\limits_y \pmodel\left(y \given[\big] x, |y| = L\right)
\end{equation*}
for a given target length, $L$.

The main thing we want to know is whether conditioning away the degenerately short outputs uncovers new issues such as disfluency and repetition, or if the length-conditional modes are high-quality.
Our main finding is that these conditional modes are indeed high-quality, provided the length constraint is long enough.
We'll mostly look at these modes qualitatively, for a more quantitative investigation of length-conditional modes, see \citet{catgotyourtongue}.\footnote{They instead condition on the length being \emph{at least} some target value, whereas we search for outputs of exactly a given length.}

One computational problem we face is that finding length-conditional modes is much harder than finding global modes.
This is because there are far fewer opportunities to prune the search tree than in unconditional search.\footnote{For finding a conditional mode of length 12, you can only prune a depth 5 subtree if it's lower probability than the best length 12 sequence found. That will rarely be the case, so you need to check more of these small trees than you would when you're searching for a global mode.}
Because of that, the highest length we targeted with conditional search was 12 tokens.

\subsubsection{Characteristics of length-conditional modes}
A common pattern in the conditional modes is that the shortest modes will not be complete sentences, but those of length 10-12 will be grammatical (while still leaving out some content by necessity).
Table~\ref{tab:marian_example} shows an example of this behavior for an input that is assigned the empty sequence as its global mode.
The length 4 mode is incomplete, but each increase in the length constraint adds more information.
The length 8 mode adds that the blast happened in Thailand, the length 10 mode adds that it was a bomb, and the length 12 one adds that it was in a tourist zone.

Table~\ref{tab:mt_modes} shows 20 more search outputs, that were randomly selected to avoid cherry-picking.
Sources A-J were randomly selected from the sequences with reference lengths between 5 and 15 tokens, so that we could search for outputs of similar length.
The problem is that the short sequences are least likely to have empty modes, so even the global modes are high quality.
Sources K-T were sampled from the sources with reference lengths between 25 and 35 tokens for which the model \emph{did} predict that the mode was empty.

\paragraph{Modes for short reference sentences.} For all the sources with short references, almost all of the length-conditional modes are grammatical.
The only strange sentence is the length 12 mode for Source G, which has spurious punctuation.
The differences in meaning from the reference translations are due to lack of details in source sentences.
Notably, the global modes for sources A, C, and D are either ungrammatical or not good translations of the source.

\paragraph{Conditional modes when the mode is empty.}
Examples K-T in Table~\ref{tab:mt_modes} show length-conditional modes for some sources for which the model predicts the empty sequence as the modal output.
Interestingly, the mode of length 12 is grammatical for 8 of the 10 sources (all but N and S).
There is no repetition, the most commonly observed other search degeneracy in beam search.\footnote{Repetition is locally super high probability: If the model outputs ``cat'' 20 times, the event that it is output a 21st time is extremely high probability. The issue is that at some point the model has to output the EOS token, which is getting lower and lower in probability the more times the repetition happens.
This makes it so that repetition can trap methods like beam search that need to make local decisions, but it doesn't actually give high-scoring full sequences.}.

The main cause of ungrammatical outputs seems to be the prescribed length being too short for all the information in the source sentence.
The reason we're stuck with this problem is that the sentences that tend to have empty model modes have reference lengths too long for us to do exact search for.
Language modeling tasks have higher entropy than MT, so we'll see empty modes at much shorter output lengths when we look at LMs in the next section.

\subsection{Discussion: Exact modes in machine translation}
Running exact search on the Marian MT Zh-En model replicated \citet{catgotyourtongue}'s finding that the unconditional mode is often empty.
On the other hand, length-conditional modes seem to generally be high quality.
The other ``degeneracy'' we see in the conditional modes is that they may be truncated when the conditioning is too short. 
That seems to be mostly due to the fact that we have to condition on lengths much shorter than the reference translations.\footnote{In the next chapter when we look at approximate search for conditional modes, we'll instead be able to condition on the length being equal to the reference length, which will fix that problem.}

Overall, we consider these findings an encouraging sign, since we didn't see repetition or disfluency in the conditional modes.
This supports our suggestion in Chapter~\ref{chapter:modes_theory} that finding the conditional argmax of a probability distribution might avoid the bad mode problem.

\section{Exact modes of a cloze completion LM}
The issue with looking at length-conditional modes of NMT models is that their output entropy rate is relatively low.
That makes it so that by the time outputs get long enough for degenerate modes to occur, they're also too long for length-conditional search to be practical.

To move to a more open-ended setting that also has outputs of tractable lengths, we used the ROC stories dataset~\citep{roc_stories}.
ROC Stories is a dataset of 5 sentence stories, where the goal is to predict the last sentence based on the first 4.
The intended way to evaluate models is to have them choose between two alternatives, but we just used it as a language modeling dataset since it has a very constrained format.
We finetuned\footnote{Hyperparameters: Adam~\citep{adam} with a learning rate of $2 \times 10^{-5}$, and a batch size of 32.} the 345M parameter GPT-2 model~\citep{gpt2} on the dataset and searched for unconditional and length-conditional completions on the validation set.
We used early stopping based on validation set perplexity over the 12 epoch training run.\footnote{This technically leaks information since we also look at modes on the validation set itself. However, we're just selecting between 12 models (1 after each epoch), which means there aren't very many bits of leakage.}

\subsection{Unconditional modes}
\begin{figure}
  \centering
  \begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/roc_frac_empty_vs_reflen.png}
    \caption{Percent of stories that have the empty sequence as their modal continuation.}
    \label{fig:roc_empty_percent}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/roc_empty_prob_tgt.png}
    \caption{Geometric mean of the model's probability of the empty sequence given the first four sentences of the story.}
    \label{fig:roc_empty_prob}
  \end{subfigure}
  \caption{Finetuned GPT-2-345M predictions of empty outputs on the ROC Stories validation set (1571 Stories). Stories are grouped into 5 equally sized bins by reference continuation length.}
  \label{fig:roc_empty}
\end{figure}
The empty sequence was the mode for 28.71\% of the 1571 ``Winter 2018'' validation set stories.
Figure~\ref{fig:roc_empty} shows that, unlike the NMT case, there's not a clear correlation between length and the probability of the mode being empty.
This is probably just due to the fact that the output lengths don't vary much.

The probability of the empty sequence averages to around 4 or 5 in ten thousand, which is quite a bit higher than in our MT experiments.
Since the ROC stories data is much cleaner than MT training data, this definitely represents model error.
The reason for it is likely just that finetuning didn't completely overwrite the base GPT-2 models' distribution of when EOT should be emitted.

\subsection{Length-conditional modes}
\begin{table}[h]
    \centering
    \caption{Modal continuations of several lengths for prefix: ``Sarah always had a fascination with the night sky. Noticing her passion, Sarah's father bought her a new telescope. She was ecstatic. She went outside every night to diligently view the night sky.'' The reference continuation is ``Sarah loved her new telescope.''}\label{tab:roc_example}
    \begin{tabular}{lll}
    Length Constraint (tokens) & Log-probability & Text\\
    \midrule
    Global mode & -7.79 & \texttt{<|endoftext|>}\\
    5 & -9.14 &  Sarah loved astronomy!\texttt{<|endoftext|>}\\
    6 & -7.97 &  Sarah never looked back.\texttt{<|endoftext|>}\\
    7 & -8.59 &  Sarah loved her new telescope.\texttt{<|endoftext|>}\\
    8 & -9.38 &  Now, Sarah is an astronomer.\texttt{<|endoftext|>}\\
    9 & -8.68 &  Sarah was happy with her new telescope.\texttt{<|endoftext|>}\\
    10 & -8.77 &  Sarah was very happy with her new telescope.\texttt{<|endoftext|>}\\
    12 & -8.91 &  Sarah was amazed by the beauty of the night sky.\texttt{<|endoftext|>}
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{Modal continuations of several lengths from a GPT2-345M model finetuned on the ROC stories corpus. The input was: ``Kaylee always wanted a puppy. On her birthday her parents took her to a farm. There were lots of beagle puppies there. Her parents told her she could pick a puppy for her birthday.'' The reference continuation is ``Kaylee was thrilled!''}\label{tab:roc_example2}
    \begin{tabular}{lll}
    Length Constraint (tokens) & Log-probability & Text\\
    \midrule
    Global mode & -6.55 &  Kaylee picked a beagle puppy.\texttt{<|endoftext|>}\\
    5 & -9.00 &  Kaylee cried.\texttt{<|endoftext|>}\\
    6 & -7.66 &  Kaylee said yes.\texttt{<|endoftext|>}\\
    7 & -6.73 &  Kaylee was so happy.\texttt{<|endoftext|>}\\
    8 & -7.25 &  Kaylee picked a black lab.\texttt{<|endoftext|>}\\
    9 & -6.55 &  Kaylee picked a beagle puppy.\texttt{<|endoftext|>}\\
    10 & -7.01 &  Kaylee picked a black and white puppy.\texttt{<|endoftext|>}\\
    12 & -7.98 &  Kaylee picked a black and white beagle puppy.\texttt{<|endoftext|>}\\
    \bottomrule
    \end{tabular}
\end{table}

Just like with the MT model, the GPT-2 model's length-conditional modes are high-quality, even when its global mode is not. Table~\ref{tab:roc_example} shows one example of this behavior. 
The mode is empty, but the length conditional modes are all plausible completions of the story, and don't display any degeneracies such as repeating earlier text from the story.

An interesting feature of these constrained modes is that the content can be correlated with the length in clear ways. Table~\ref{tab:roc_example2} shows an example where the mode of length 5 is significantly different from all the other modes.
It may be impossible to produce a 5 token output that has the right content, but the model ``prefers'' to output something grammatical, so we see different content.
This is different from the short NMT modes, which were often truncated when the constraint was too short to express the content of the source sentence.

In order to show that these patterns aren't just cherry-picked, randomly sampled examples of modal outputs are shown in Table~\ref{tab:roc_modes}.
All 30 of the conditional modes are grammatical, relevant to the context, and don't show any evidence of degenerate behavior.
This is further evidence that conditional MAP inference may be a promising direction of investigation.

\subsection{Discussion: Exact modes for cloze completion}
Our findings for this finetuned GPT-2-medium model were essentially the same as what we found for the MT model.
Specifically, the empty sequence is often the modal output, but conditioning on a desired length can yield better results.
The length conditional modes are essentially always grammatical, unlike for the MT model where they were often truncated for shorter target lengths.
This is probably because we were able to condition on lengths that were similar to the length of the actual reference continuations, which was not the case for our MT experiments.

To our knowledge, this is the first time exact and conditional modes have been investigated for a language model, so this generalizes the prior findings of \citet{catgotyourtongue}.
A priori, we were worried that length-conditional modes from GPT-2 might just be a single word repeated over and over, or a repetition of an earlier sentence from the context.
The fact that they're high-quality even for this open-ended task is extremely encouraging.


\section{Exact modes of LLaMA-based models}
The earlier experiments replicated~\cite{catgotyourtongue}'s results, and extended them from MT models to a language model as well.
The length-conditional search results showed that these models' modes are usually high-quality, as long as the length is constrained to an appropriate value.

However, those experiments used models that are much smaller than modern LLMs, as well as the LM experiment using a synthetic task (no one actually wants a model that adds a 5th sentence to 4 sentence stories).
To extend our work to a more realistic setting, we also run exact search on three variants of the 7B parameter LLaMA model~\citep{llama} using prompts from the \texttt{databricks-dolly-15k} dataset~\citep{dolly15k}.
The three models are: the base LLaMA-7B model, Alpaca 7B~\citep{alpaca}, and Guanaco-7B~\citep{qlora}.
LLaMA is trained as a general language model, while the other two are finetuned from it on instruction following specifically.

Since these models are over 10 times larger than the models in the previous sections, we only run exact mode search and not length-conditional mode search.
The goal of examining this modes is to verify the assertion that ``the bad mode problem won't go away with scale or improved training'', from Chapter~\ref{chapter:modes_theory}.

\subsection{Details of mode search for LLaMA-family models}
We sampled 1000 instructions from the \texttt{databricks-dolly-15k} dataset, filtered to be less than 256 tokens long, and to be in the instruction/response format rather than the instruction/context/response format.
For Alpaca and Guanaco, we use the prompt format used during finetuning, but LLaMA isn't trained for instruction following so we just use the Alpaca format for it as well (See Appendix~\ref{chapter:prompts_appendix} for the exact text).

We ran DFS on the same set of inputs for each of these models, using the caching strategy we described in Section~\ref{sec:modesexact_dfs_mem}.
One issue is that Guanaco was trained on multi-turn conversations, which means it will generate more messages instead of outputting EOS.
To fix that we treat ``\texttt{\textbackslash{}n\#\#\#}'' as an alternative EOS marker in addition to \texttt{</s>}, which prevents it from generating more than one message.

\subsection{Quantitative Results}
\begin{table}[h]
    \centering
    \begin{tabular}{lrr}
        Model & \% modes empty & $P(\text{empty})$\\
        \midrule
        LLaMA & 70.7 & $1.13 \times 10^{-4}$\\
        Alpaca & 16.0 & $1.80 \times 10^{-5}$\\
        Guanaco & 7.70 & $2.48 \times 10^{-6}$\\
    \end{tabular}
    \caption{Statistics of 7B parameter LLaMA variant models' predictions of empty modes.}
    \label{tab:llama_empty_stats}
\end{table}

\begin{figure}
  \centering
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/llama_frac_empty.pdf}
    \caption{Percent of prompts for which each model's modal response is the empty sequence.}
    \label{fig:llama_empty_percent}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/modes/llama_empty_probs.pdf}
    \caption{Difference between the average base-2 log-probability of the empty sequence for a particular reference length decile, and the average over all reference lengths.
    This relative view is to put all the log probabilities in the same range, see Table~\ref{tab:llama_empty_stats} for the absolute values.}
    \label{fig:llama_empty_prob}
  \end{subfigure}
  \caption{LLaMA 7B, Alpaca 7B, and Guanaco 7B predictions of empty outputs on 1000 prompts from the \texttt{databricks-dolly-15k} dataset. Prompts are grouped by the decile of the length of the reference response.}
  \label{fig:llama_empty}
\end{figure}

\begin{figure}[htbp]
  \centering

  % First subfigure (side by side)
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{figures/modes/alpaca_mode_logprob_vs_mean_sample_logprob.pdf}
    \caption{Alpaca}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{figures/modes/guanaco_mode_logprob_vs_mean_sample_logprob.pdf}
    \caption{Guanaco}
  \end{subfigure}

  % Second subfigure (centered below)
  \begin{subfigure}{0.6\linewidth}
    \includegraphics[width=\linewidth]{figures/modes/llama_mode_logprob_vs_mean_sample_logprob.pdf}
    \caption{LLaMA}
  \end{subfigure}

  \caption{The log-probability of the modal (y-axis) output compared to the mean log-probability of 5 samples for each of 1000 prompts from the \texttt{databricks-dolly-15k} dataset. Empty modes tend to only occur for lower sample-logprob (higher-entropy) inputs for Alpaca and Guanaco. The 5\% of points with the lowest ``Mean sample logprob'' values have been truncated for readability.}
  \label{fig:sample_logprobs}
\end{figure}
% Plots to add: Frac empty vs sample logprob

Just like with the smaller models, all three of the LLaMA model variants often have an empty modal output.
Table~\ref{tab:llama_empty_stats} shows the percent of prompts that cause each model to predict an empty mode.
LLaMA has an empty mode more than 4 times as often than the other two models, which isn't surprising, since Alpaca and Guanaco were trained on data where the LM always gives a full response to the user.

Figure~\ref{fig:llama_empty} shows the same pattern happens with LLaMA as in the earlier experiments: Inputs with longer reference lengths have empty modes more often, but the probability of empty outputs either declines or is relatively unchanged with length.
In Figure~\ref{fig:llama_empty_prob}, Alpaca is the only model that shows a clear trend in terms of empty probability, but even it only changes by a factor of about $2 / 2^{-0.45} \approx 3$.

As mentioned in Chapter~\ref{chapter:modes_theory}, it's commonly thought that the bad mode problem occurs when a task is less-constrained (meaning there are many correct responses).
We don't have access to multiple references, but we can estimate how spread the \emph{model}'s estimate of output distribution is, then see how that relates to mode emptiness.

Figure~\ref{fig:sample_logprobs} shows this relationship, by showing (for each prompt) the logprob of the mode, the average logprob over 5 samples\footnote{The average log-probability of a sample is just the entropy, so this is an estimate of the negative conditional entropy for a prompt. A lower value means that the model's distribution is more spread out for that prompt.}, and whether the modal output is empty.

The Alpaca and Guanaco modes support the ``level-of-constraint'' hypothesis, with the empty modes only occurring when the estimate of the entropy is below some threshold.
LLaMA, on the other hand, has empty modes even for prompts with fairly low entropies (high sample logprobs).
Emitting an EOS token right away is an error for the Alpaca and Guanaco training tasks (conversation/QA), but could actually be correct for the web data LLaMA was trained on.

\subsection{Qualitative analysis: Which prompts lead to empty modes?}
Instruction-following is a much more varied task than either MT or story completion, in terms of how constrained the set of responses is.
In MT, we'd expect that the entropy of the output roughly scales with the input length.
With instruction-following, it's easy to come up with short inputs that have extremely high output or extremely low entropy.

In Chapter~\ref{chapter:modes_theory}, we suggested that the bad mode problem shouldn't be thought of in terms of length, but in terms of the entropy of the set of valid outputs.
This is often related to length, but can easily be decoupled from it.
For example, when prompted with ``Recite the Declaration of Independence.'', Alpaca's global mode is the first 151 tokens of the preamble, ending with ``\ldots to effect their safety and happiness.''
On the other hand ``Write a brief paragraph of the benefits of attending Arizona State University'' is assigned the empty mode.
The latter prompt has many valid outputs shorter than 151 tokens, but the entropy of those valid outputs is clearly \emph{far} higher than the entropy of the set of valid responses to the recitation prompt.

In the previous section, we quantitatively looked at the relationship between open-endedness and empty modal outputs.
Here, we also look at it quantitatively by giving more examples of prompts that lead to empty or non-empty outputs.
Tables~\ref{tab:alpaca_empty_prompts}, \ref{tab:guanaco_empty_prompts}, and \ref{tab:llama_empty_prompts} show 10 of each for each of the three LLaMA-based models, which were randomly sampled to avoid cherry-picking.

For Alpaca and Guanaco, the prompts that have empty modes are generally asking much more open ended questions, which don't have a single clear answer.
Most of the prompts for which LLaMA has a non-empty mode are factoid requests that have a single answer.

\subsection{Qualitative analysis: When the mode is non-empty, is it degenerate?} We observe that when these models' modes are non-empty, they are often high-quality, although we do see problems that weren't present with the models trained on more constrained tasks.

Tables~\ref{tab:alpaca_modes}, \ref{tab:guanaco_modes}, and \ref{tab:llama_modes} show the model modes for the prompts that have non-empty modes.
While some modes are correct responses, there are also degenerate behaviors besides empty outputs.
We'll briefly summarize the issues here.

\paragraph{Alpaca:} Nine of the ten Alpaca outputs are high quality, but Alpaca Prompt I has the output ``\textless{}nooutput\textgreater{}'' which is a tag appearing 28 times in the 52,000 Alpaca training examples.
This exact string was the mode for 46 out of the 1,000 prompts we searched.

\paragraph{Guanaco:} Eight of the modes are high quality (albeit with some factual errors), but Guanaco prompts B and G lead to a mode which is just a phrase from the prompt instead of an answer.
It's hard to measure how often that happens \emph{and} is undesirable, since many of the Dolly prompts require an answer which is part of the prompt.

\paragraph{LLaMA:} Prompts B, E, F and J repeat all or part of the prompt rather than responding.
In general all of these modes are very short, but that isn't surprising since 70\% of LLaMA modes are empty overall.
The prompts that \emph{do} have non-empty modes will tend to be ones that can be answered very concisely.

These modal outputs show that for these LMs, there are multiple types of degenerate outputs.
This is different from the situation with the ROC stories LM or NMT model, where the empty mode seemed to basically be the only problematic mode.

Addressing this problem will be harder than just conditioning on a single deterministic property like length.
For example, when we re-ran exact search on LLaMA-7B, but blocked the empty output from being produced, 17.2\% of the modal outputs were the string ``\textbackslash{}end\{code\}''.
All the above issues \emph{could} be addressed by heuristic modifications to search, but those heuristics have issues:
\begin{enumerate}
    \item \textbf{Short/Empty outputs.} One option is to maximize logprob per token instead of the overall probability, but repetition of strings from the prompt will have high probability. Also, extremely long strings of one token repeated many times have extremely high logprob per token, since if you've said the word ``hello'' 500 times, the probability of saying it again is very high.
    \item \textbf{Repetition of prompt.} Direct ngram blocking can help, but as we mentioned in many cases repeating parts of the prompt is desirable. One common use case of chatbots is for proofreading, which often requires repetition of large amounts of text.
    \item \textbf{LLaMA's Love of LaTeX.} When specific substrings like ``\textbackslash{}end\{code\}'' are degenerate modes, we can prevent them from being produced, but there might be a large number of such outputs, and of course there's also the problem that they might sometimes be the appropriate response.
    A harder example of this same problem is the ``safety'' outputs that many current chat models produce, where they refuse to answer a request.
    Since the refusal texts are low entropy, they might be modal even when the model thinks there's a 1\% chance it should refuse.
\end{enumerate}

As we said in Chapter~\ref{chapter:modes_theory}, what we really want is to be able to search for the output, $x$, that maximizes:
\begin{equation*}
    \prob \left(x \given[\big] \text{``$x$ is a well-formed response to the prompt''}\right)
\end{equation*}
Doing exact search on that objective is probably intractable, for basically any definition of ``well-formed.''
In the next chapter we investigate how to approximate search of this kind using beam search.

\section{Conclusion}
In this section we looked at the exact modes of NLG models in three settings: Chinese-to-English machine translation, story cloze completion, and instruction-following.
We reproduced the results of \citet{catgotyourtongue}, and extended them to a GPT-2 based LM, as well as three LLaMA-based LMs.

For MT and cloze completion, we found that searching for \emph{length-conditional} modes instead of unconditional modes usually produces high-quality outputs.
This is encouraging, since prior work (See Section~\ref{sec:modestheory_related_work}) had identified that model likelihood often diverges from quality past some point.
These results provide support for the hypothesis we proposed in Chapter~\ref{chapter:modes_theory}: There may be low-quality outputs that are low-probability in absolute value, but due to the high entropy of the set of valid outputs, they still become the mode.
Our finding for MT that the empty output receives a lower probability for longer inputs, but is also \emph{more} likely to be the mode for those inputs is exactly what we would predict based on our reasoning in the last chapter.

We also found that, apart from empty modes, the LLaMA-based language models often have high-quality modes, but sometimes fall into new problems such as repeating their prompt.
In the next chapter, we take advantage of these findings to improve outputs from LLaMA-7B using beam search.

==> modes/llama_beams.tex <==
How are odds different from probability? & Probability is a measure of the likelihood that an event will occur. Odds are a measure of the likelihood that an event will not occur. & Probability is a number between 0 and 1 that represents the likelihood that an event will occur.\\
Which author created Dick Tracy & Al Capp & Al Capp\\
What is a web browser? & A web browser is a software application for retrieving resources over the World Wide Web. & A web browser is a software application for retrieving, presenting, and traversing information resources on the World Wide Web. An information resource is identified by a Uniform Resource Identifier (URI/URL) and may be a web page, image, video, or other piece of content. Not all web browsers are general-purpose; e.g. mobile browsers are built specifically for mobile devices.\\
Why do people like cats? & People like cats because they are cute and cuddly. & People like cats because they are cute.\\
What is the difference between a GPU and a CPU? & A GPU (Graphics Processing Unit) is a special-purpose processor designed to accelerate the rendering of 2D and 3D computer graphics. A CPU (Central Processing Unit) is the part of a computer that carries out the instructions of a computer program by performing the basic arithmetical, logical, and input/output operations of the system. & A CPU (Central Processing Unit) is the "brain" of a computer, while a GPU (Graphics Processing Unit) is the "eyes" of a computer.\\
What is Passover? & Passover (Hebrew: [\ldots], Pesach) is a Jewish holiday commemorating the Exodus from Egypt. Passover begins on the 15th day of the Hebrew month of Nissan and lasts for either seven days (in Israel) or eight days (in the Diaspora). & Passover is a Jewish holiday that celebrates the liberation of the Israelites from slavery in Egypt.\\
Give me a bulleted list of 5 states in alphabetical order & Alabama, Alaska, Arizona, Arkansas, California & Alabama, Alaska, Arizona, Arkansas, California\\
Why do some countries outperform other countries in certain sports despite having a smaller population? & \texttt{<empty>} & The answer to this question depends on what you mean by "outperform". If you mean "win more medals", then the answer is simple: more medals are won by countries with a larger population. If you mean "win more medals per capita", then the answer is also simple: more medals are won per capita by countries with a smaller population.\\
Summarize the Challenger Sales Methodology for me & \texttt{<empty>} & The Challenger Sale: Taking Control of the Customer Conversation, by Matthew Dixon, Brent Adamson, and Pat Spenner, published by Harvard Business Review Press, 2011.\\
What is the Azure equivalent of EKS? & There is no Azure equivalent of EKS. & The Azure equivalent of EKS is Azure Kubernetes Service (AKS).\\
Who wrote The History of Mr Polly & The History of Mr Polly was written by H. G. Wells. & The History of Mr Polly was written by H. G. Wells.\\
Write a tweet from the perspective of a dog that’s angry about the squirrels in its yard & \texttt{<empty>} & SQUIRRELS HAVE TAKEN OVER MY BACKYARD AND I’M NOT HAPPY ABOUT IT\\
What are the advantages and disadvantages of allowing people to perform delivery tasks by walking instead of requiring the use of a bike or car? When do you think it is more pragmatic for deliveries to be fulfilled by walking versus biking or driving? & \texttt{<empty>} & Walking is the most pragmatic way of fulfilling deliveries, as it is the most cost-effective and environmentally-friendly way of fulfilling a delivery. Walking is the most cost-effective way of fulfilling a delivery, as it does not require any fuel or electricity to fulfill a delivery. Walking is also the most environmentally-friendly way of fulfilling a delivery, as it does not release any carbon dioxide into the atmosphere when fulfill\\
What are good native plants for a garden in Ohio? & \texttt{<empty>} & The best native plants for a garden in Ohio are those that are native to Ohio.\\
Identify which animal species is alive or extinct: Velociraptor, Pacific Salmon & Velociraptor & Velociraptor, Pacific Salmon\\
Who is the Disney character named Grogu? & Grogu is a character from the Star Wars franchise. & Grogu is not a Disney character.\\
Identify which animal species is alive or extinct: Stupendemys, Gray Whale & Stupendemys is extinct. Gray Whale is alive. & Stupendemys\\
What field of science (biology, physics or chemistry) was Marie Curie a researcher in? & Marie Curie was a researcher in chemistry. & Marie Curie was a researcher in physics and chemistry.\\
Which of these are woodworking handtools: plane, spokeshave, drill, table saw, chisel, bandsaw & \textbackslash\{\}begin\{itemize\}\textbackslash{}n\textbackslash\{\}item plane\textbackslash{}n\textbackslash\{\}item spokeshave\textbackslash{}n\textbackslash\{\}item drill\textbackslash{}n\textbackslash\{\}item table saw\textbackslash{}n\textbackslash\{\}item chisel\textbackslash{}n\textbackslash\{\}item bandsaw\textbackslash{}n\textbackslash\{\}end\{itemize\} & A plane, a spokeshave, a drill, a table saw, a chisel, a bandsaw\\
Tell me a romantic fact about animals. & A romantic fact about animals is that they can be romantic. & There are no romantic facts about animals.\\
\bottomrule


==> modes/theory_chapter.tex <==
\chapter{Degenerate NLG outputs might not be due to model error}\label{chapter:modes_theory}
While the previous chapters have focused on transformer language models, in this chapter we will be discussing issues which affect all language models, in the sense of models which represent distributions over text.
We give a mix of new ideas, and ones which have been discussed in prior work, with the goal of encouraging the NLP community to think more closely about the issue of degenerate NLG outputs such as those identified by \citet{catgotyourtongue}.
We will start with a motivating analogy.

\subsubsection{Predicting the future with a TV}
Imagine you were watching a TV, and you wanted to predict what the next frame would be, based on the current frame.\footnote{Bear with us, we'll get back to NLP momentarily.}
If you had infinite training data, time, and compute, you'd eventually be able to do as well as possible at this task.

``As well as possible'' might not be perfect.
Realistically, there will be \emph{intrinsic uncertainty} in distribution of next frames.
Intrinsic uncertainty occurs when there are multiple possible outputs for a given input.
If the input is a picture of a baseball suspended in mid air, you might not be able to perfectly guess the next frame, since you don't know which way the ball is flying.
Even worse, it's possible that at any time, the feed will cut from one scene to another.
You'll have to train a model which represents this uncertainty.
That is, given a current frame $x$, your model will tell you $\prob(y | x)$ for any possible next frame $y$.

This model by itself isn't enough, you want to predict the next frame, not just know how likely each frame is.
The process of mapping from an entire distribution to a single prediction is called \emph{decoding}, and there are many different ways to do it.
There are at least two obvious strategies, which we'll refer to as \emph{sampling} and \emph{search}, as they're stand-ins for more general classes of methods.
The sampling strategy is to draw a single sample from the probability distribution your model learned.
The search strategy is to predict the single frame which the probability distribution thinks is most likely.
This particular search strategy is called \emph{maximum a posteriori} (MAP) decoding.

To make your job a bit harder, imagine the TV has a damaged cable which adds noise to the incoming data.\footnote{To be specific let's imagine that each frame is corrupted by additive spherical Gaussian noise in pixel space.}
If you trained your model on these noisy inputs, there'd now be a noticeable difference between sampling and search.
Sampling would usually give you an output which has the same amount of noise as an average image, but search would probably give you a noise free image.\footnote{This might not be true if the distribution of images conspires against you, but for a low enough noise scale it will be.}
Your model knows enough about the data distribution to ignore the noise, and give you a clean frame.

You really want to know what happens in the next frame of the TV program, so you decide to go with search instead of sampling.
Now let's make things even worse, and suppose that on top of the additive noise, 1 in 1,000 frames gets dropped altogether.
When this happens, your TV just shows a black screen, with no image or even the noise.

Now we have a real problem.
If the distribution of noise-free images consists of more than 1,000 images which are all equally likely, any individual \emph{real} next frame will be lower probability than the blank screen!
Realistically, there are likely \emph{far} more than 1,000 similarly likely outputs, so the probability of the blank frame could be even smaller, and this problem would still occur.
When both the frame corruption \emph{and} the frame dropping noise are present, neither search nor sampling will give you a good output.
Sampling will give you noisy images, and 1 in 1,000 times it will give a blank output.
Search, on the other hand, will just give you a blank screen every time.

The problem here isn't in your model; it fits the data perfectly!
The problem is your decoding methods, which are vulnerable to the two types of noise in video stream.
Your model still knows what the  most likely non-noise frame is, and you can extract it by looking for the mostly likely frame which isn't blank, i.e.:
\begin{equation*}
    y_\text{pred} = \argmax\limits_{y} \prob \left( y \given[\big] x, \text{ ``$y$ is not blank''}\right)
\end{equation*}
This decoding method just extracts a \emph{conditional mode} instead of the unconditional mode.

\subsubsection{Relationship to NLG}
We will argue that the TV prediction game above is closely analogous to decoding from models in NLG.
In particular, we use decoding methods which are susceptible to specific types of noise in our datasets, then blame it on our models when those decoding methods give us low quality outputs!

This claim is primarily based on empirical and theoretical arguments which have already been made in the NLP literature.
For example, \citet{catgotyourtongue} in particular found that NMT models predict that the empty sequence is the modal translation for many inputs.
However, these findings are often assumed to be evidence of \emph{model error}.
The reason for this chapter is to try help the NLP community build intuition about this topic, as well as suggesting possible ways to handle noisy distributions.
We'll focus in particular on the ``bad mode problem'', the issue that NLG models will often assign a higher probability to degenerate outputs than good ones.

The important thing to understand about this chapter is that it is about \emph{sequence distributions}, as opposed to models trained on them.
So, if we convincingly argue that a distribution has some problem, it implies that no amount of improvements in model training can fix that issue.
The question is then whether the training data distribution itself has that problem.
We will argue that it is likely that real text corpora \emph{do} have noise modes which lead to undesired outputs.

The rest of this chapter consists of the following:
\begin{itemize}
    \item Section~\ref{sec:modestheory_notation} introduces notation for the rest of the chapter, and formalizes the issue we see with decoding methods via an ``oracle criterion.''
    \item Section~\ref{sec:modestheory_related_work} goes over past empirical findings on the bad mode problem, as well as how those findings have been interpreted.
    \item Section~\ref{sec:modestheory_examples} gives several examples of sequence distributions which display the bad mode problem.
    \item Section~\ref{sec:modestheory_realistic} argues that this phenomenon might be present in the distributions of our actual training sets as well.
    \item Section~\ref{sec:modestheory_proposal} discusses possible approaches for decoding from noisy distributions.
\end{itemize}
Chapter~\ref{chapter:modes_exact} will extend this by looking at the exact modes of several NLG models.

\section{Data distributions and the oracle criterion}\label{sec:modestheory_notation}
As we indicated in the introduction, many common decoding methods will produce undesirable results when used on distributions which contain noise.
To make this more concrete, we propose that we should reason about decoding algorithms in terms of how they behave when applied to the \emph{training distribution itself}.
Since we don't have access to the actual training data distribution, only a finite sample of it, we are only recommending this as a fruitful kind of thought experiment, not an empirical test.
In Section~\ref{sec:modestheory_examples} we'll apply this method by looking at the exact mode of a number of sequence distributions.

In the rest of this section we'll introduce some notation, and make the connection between the television example and NLG more explicit.
We'll then make the idea of decoding directly from the training distribution more concrete as the \emph{oracle criterion}.

\subsection{Notation}
\paragraph{The set of outputs} In all of our settings, we have some outputs which we want to predict, usually based on some inputs. We'll refer to the set of all possible outputs as $\seqs$. In the TV example $\seqs$ would be the set of all possible pixel assignments for our TV screen, while in the rest of the section it will be the set of all finite sequences from a vocabulary.

\paragraph{The ``clean'' subset.} The thing we really care about is outputs which are correct for a given input, which we'll call $\sperfect$.
When we need to specify that it depends on a particular input, $x$, we'll write $\sperfect(x)$.
(This generalizes to the case of unconditional generation by considering a single constant input).
In the TV example, for a previous frame $x$, $\sperfect(x)$ consists of frames which could follow $x$ in the absence of noise.
An example from NLP would be the set of valid translations for an MT task:
\begin{equation*}
    \sperfect(x) = \{y | y\text{ is a translation of }x\}
\end{equation*}
Note that this depends entirely on some task-specific notion of quality or correctness.
Consider the task of replying to Reddit comments.
If the goal is to simulate a Redditor, $\sperfect(x)$ includes all comments which might be replies to $x$.
On the other hand, if the goal was to give \emph{helpful} replies, $\sclean(x)$ would not include things like jokes, insults, etc.

\paragraph{The clean distribution.} We'll write $\dperfect$ for a distribution only supported on $\sperfect$.
This would be the distribution of next frames only including intrinsic uncertainty and no noise in the TV analogy.
In the task of summarization, for example, $\dperfect$ should be a distribution over all valid summaries of the input.

\paragraph{The training distribution.} For a distribution which potentially contains some noisy outputs, we'll write $\dtrain$. The noise could be due to $\dtrain$ being a mixture between $\dclean$ and some noise (as with the blank frames in the TV example), or due to corruption of outputs (the additive noise in the TV example).
In NLP this is the population distribution for a training set, including whatever noise is present.
We'll write $\ptrain(\cdot)$ for the probability that an event occurs under $\dtrain$, or the PMF of a random variable when the argument is a random variable.

\paragraph{Attributes.} We don't just want to view all texts as identical, so we'll need some way to categorize them.
We'll talk about \emph{attribute functions}, $A(x)$, which map an output $x$ to an set of possible values $\mathcal{A}$. For example, in our TV setting we might have $A(x)$ return the truth value of ``x is a blank frame''. One we'll make a lot of use of is length, so $A(x) = |x|$ and $\mathcal{A} = \mathbb{N}$.
Other examples include ``Is $x$ a fluent text?'', or ``Does $x$ have positive sentiment?''
These attributes are binary, so $\mathcal{A}$ would be the set $\{0, 1\}$.

\subsection{The oracle criterion}
We want to encourage the community to think more rigorously about what NLG behaviors are due to model error, and which are due to the difference between $\dtrain$ and $\dclean$.
If low-quality outputs are due to noise in the training data, we need to get better data or improve our decoding.

For analyzing decoding methods, we propose the following criterion:
\begin{mdframed}[backgroundcolor=gray!10, linewidth=0pt, innertopmargin=10pt, innerbottommargin=10pt]
    \textbf{Oracle Criterion:}\\
    An NLG decoding method should produce high-quality results if it is applied to the relevant oracle for $\dtrain$.\footnote{Different methods may need different oracles. For example, ancestral sampling needs the next token distribution $\ptrain(x_{t} | x_{<t})$. Non-autoregressive sampling methods may need $\ptrain(x_{t} | x_{<t}, x{>t})$.}
\end{mdframed}
Informally, the point is that if a decoding algorithm can't produce good outputs even when a model is trained perfectly, we should use a better method.

It may still be the case that we want to use methods which would not work well on $\dtrain$ in order to compensate for model error.
For example, nucleus sampling excludes the tail of the token distribution, which probably helps due to our models not accurately fitting that part of the text distribution.
However, we should be explicit about which of our decoding choices are made to compensate for model error, and would be necessary regardless of how well the model is trained.

\section{Prior empirical findings}\label{sec:modestheory_related_work}
In this section we'll look at past results related to the bad mode problem, as well as what the authors inferred from their findings.
Each of the snippets below is just the findings/claims from each paper which are directly applicable, not a full summary.

The repeated points are that on some (but not all) tasks NLG outputs can be high-likelihood while still being low quality.
The issue is generally attributed to some kind of model error or bias, and findings generally indicate that it gets worse on tasks where outputs are less constrained (although no one agrees on what measure of constraint to use).

\subsection{\citet{catgotyourtongue}}
\paragraph{Findings:} The authors ran exact MAP inference for a transformer MT model on the WMT \texttt{news-test2015} dataset.
They found that the empty sequence was the modal for 51.8\% of inputs, and were the first to report this kind of result.
On top of that, longer source sentences were \emph{more} likely to have the empty sequence as the modal output.

\paragraph{Interpretation:} They described these results as ``serious NMT model error,'' and ``evidence of NMT’s failure to properly model adequacy.''
More specifically, they say that ``at the root of the problem lies an inherent bias towards shorter translations.''

\subsection{\citet{inadequacyofmode}}
\paragraph{Findings:} Eikema and Aziz pointed out that \emph{samples} from NMT models don't have the same degeneracies as MAP or beam search outputs.
They found that samples were closer to the reference translations in terms of both length and n-gram statistics.
\paragraph{Interpretation}: They call the mode \emph{inadequate}. Specifically, they say: ``The mode often does not represent any significant amount of probability mass under the learnt distribution. We therefore argue that MAP decoding is not suitable as a decision rule for NMT systems.''
They also say that to criticise a model reasonably, you have to view it as an entire distribution instead of just looking at the mode.

This is a point we completely agree with them on, but our reasoning is different.
The reason they give is: ``the most likely translations under the model accumulate so little probability mass that the mode can be considered essentially arbitrary.''
We won't disagree with that, but we'll instead look at what causes bad modes to occur, and whether we can get any use out of MAP-type methods despite them.

\subsection{\citet{josifoski-likelihood-utility}}
\paragraph{Findings:} Josifoski et al. looked at the relationship between model-likelihood and utility of output across several NLG tasks and decoding methods.
They found that likelihood and utility were positively correlated for information extraction, but when using for machine translation, they were mostly negatively correlated.
For the other tasks, there were only weak correlations.

\paragraph{Interpretation:} They give a taxonomy of possible sources of disagreement between likelihood and utility:
\begin{itemize}
    \item \textbf{Training imperfections (TI)}: ``The model is trained on a different objective than the true utility, because of the finite size of the dataset and the approximation error in training''
    \item \textbf{Distribution shift (DS)}: ``When the training and testing distributions differ''
    \item \textbf{Utility drift (UD)}: ``UD occurs when the notion of utility changes, i.e. the labels for the same data points are changing.''
\end{itemize}
For example, they list NMT as a task where TI and DS are present, but UD is not.
They conclude that TI alone is present, likelihood is a strong predictor of utility, but when DS/UD are present this is not the case.

\subsection{\citet{riley2022continuum}}
\paragraph{Findings:} Riley and Chiang create a spectrum NLG tasks with varying levels of constraint by training NMT models using partially incomplete source sentences.
Training with 0\% of the source is just language modeling, using 100\% is MT, and other values give new tasks which are partially constrained.
For lower constraint levels, they say: ``beam search decoding that is too short, greedy-decoding which is too long and repetitive, and random samples that are disfluent.''
When they increase the level of constraint, length bias and repetition both improve.
\paragraph{Interpretation:} They point out that a unigram LM would have the same three problems as they found in beam search, so they say insufficient context-sensitivity might be the cause.

\begin{comment}
They consider whether output distribution entropy is a good way to predict when
In order to investigate whether output distribution entropy is the right way to formalize ``level of constraint'' they try training models with label smoothing.
It doesn't lead to \footnote{Note that this is for beam search, which may not have its output changed even if the global mode changed. \citet{liang2022implict} showed that label smoothing necessarily puts an upper bound on the length of the modal model output for example.}
\end{comment}

\subsection{\citet{nucleus_sampling}}
\paragraph{Findings:} Using beam search with GPT-2 produces repetitive outputs.
The authors also look at the per-token probability of beam-search generated and human text and find that the human text has much lower probability per token, and much more variation in probability between tokens.
\paragraph{Interpretation:} They argue that probability maximization is not appropriate for open-ended generation, as humans are not trying to output maximally probable sentences.

\subsection{\citet{zhang2021trading}}
\paragraph{Findings:} Using samples from GPT-2-774M~\citep{gpt2}, Zhang et al. observe that likelihood is correlated with crowdworker-rated quality up until a point, and negatively correlated afterward.
They also draw many samples across multiple hyperparameter settings for three sampling methods: temperature, top-k~\citep{topk}, and nucleus sampling.
When the settings are such that the decoding methods have similar output entropies, all methods perform similarly.
The exception is that nucleus sampling performs best when entropy is very low.
\paragraph{Interpretation:} The authors don't speculate about the source of the reversal in likelihood/quality correlation.

\subsection{\citet{wiher2022ondecoding}}
\paragraph{Findings:} They evaluate many decoding methods on several different NLG tasks.
The decoding methods are: greedy search, beam search, diverse beam search, pure sampling, top-k sampling, nucleus sampling, and Minimum Bayes Risk (MBR).
The tasks are MT, abstractive summarization, dialogue, story generation, and unconditional generation.
In general, beam search variants perform best for the tasks which have some constraint: MT, summarization, and dialogue.
For story generation, and unconditional generation, the sampling based methods perform best.
They find that for MT and summarization, quality and probability are positively correlated, while this relationship is flipped for story generation and unconditional generation.\footnote{This doesn't contradict other findings about high-likelihood/low-quality sequences in MT since none of the decoding methods can find super high-likelihood sequences.}
\paragraph{Interpretation:} Since the performance of decoding strategies varied so strongly between tasks, they say ``Practitioners should take great care in basing their choice of decoding strategy off of results reported for alternate tasks.''

\subsection{Summary}
One repeated finding is that likelihood-maximization based approaches tend to work less well for tasks that are less constrained.
Also, many authors indicated that the degeneracies they found are likely due to model error.
To be clear, this isn't a central point of their arguments, it's just the default assumption when we observe behavior like this.
\citet{inadequacyofmode} in particular argued that MAP was a poor decoding strategy, but their reasoning was that the mode is too small of a fraction of an MT model's output distribution.
This may also play a role in the bad mode problem, but in the next chapter we'll actually see that \emph{conditional modes} are often high quality, meaning that the low probability of the mode can't be the whole story.

\begin{comment}
OLD INTRO
In this chapter I will argue that widely observed degeneracies in LM and MT outputs do not necessarily imply that a model is imperfectly trained.
The goal is to remind the NLP community of certain facts about sequence distributions and what their implications are for analysis of past results as well as future research into decoding algorithms.

The core issue is that natural language generation (NLG) models often assign high probabilites to sequences which are low quality.
This was dramatically demonstrated by \citet{catgotyourtongue}, who found that NMT systems often assign the empty sequence a higher score than \emph{any} other translation of a given source sentence.

In general, probabilistic models of language often have the property that their most preferred (i.e. modal) text is degenerate in some way.
We will refer to this issue as the ``bad mode problem.''
Length degeneration is the most commonly observed issue, but we will give examples of other undesirable qualities that can occur.

When beam search is introduced, the intractability of exact search is often given as motivation, and it intuitively seems that increasing the beam size should be a way to trade off latency for quality.
However, exact search is actually tractable (this is how ~\citet{catgotyourtongue} got their results), merely expensive.
In fact, beam search seems to be in a middle ground between samples and exact search which has desirable properties (See ~\citet{meister-etal-2020-beam} for investigation of this).
So while one can find higher likelihood sequences by increasing the width of the beam, the bad mode problem makes it undesirable.

The bad mode problem is frequently cited as evidence of \emph{model error} or bias, that is a mismatch between the population distribution $\dpop$ and the learned distribution, $\dmodel$. (See for example \citet{catgotyourtongue}, \citet{josifoski-likelihood-utility}, \citet{murray-correcting-length-bias}).
In this chapter I will argue that this is not necessarily the case.

\begin{displayquote}[Claim 1]
Even a perfectly trained model can exhibit the bad mode problem
\end{displayquote}
Claim 1 is shown to be true in Section~\ref{sec:modestheory_examples}.
It is not exactly novel, as the difference between modal and typical sequences has been explored before (e.g. \citet{inadequacyofmode,typical_sampling}).
This framing, however, hasn't been fully internalized by the NLP community.
In particular, in order for low-quality modes to imply the existence of model error, one needs to know that the population data distribution is not similar to any of the examples given in Section~\ref{sec:modestheory_examples}.

That brings us to a second claim:
\begin{displayquote}[Claim 2]
   Real data distributions plausibly have bad modes 
\end{displayquote}
In Section~\ref{sec:modestheory_realistic}, I will describe how tiny amounts of noise in an NMT dataset could cause the bad mode problem to occur, even for a perfectly trained model.
If Claims 1 and 2 are both true, then no amount of improved training will ever fix the bad mode problem.

\begin{displayquote}[Criterion name here]
An NLG decoding method should yield high quality outputs if it were applied to the relevant oracle for the population data distribution, namely $\ppop(\xcurr | \xprev)$ for the autoregressive case.
\end{displayquote}
Consider an oracle which could, given a source sentence $x$, tell you the probability the event ``A reference translation of $x$ created by the process that generated the europarl training set has $y_{1:t}$.''
This is the probability distribution we are training our NMT models on (modulo possible label smoothing).

It's likely that none of the standard decoding methods would actually let us extract high quality translations from this oracle (See Section~\ref{sec:modestheory_realistic}), so we should look for new methods!

An alternative strategy is to either train our models for a different target, such that our decoding methods \emph{will} work.
This is what label smoothing does, allowing beam search to produce better outputs at the cost of degrading the distribution.

In this chapter I'll first go over several of the empirical findings which demonstrate the problem, as well as the interpretations/explanations that were given.
In Section~\ref{sec:modestheory_examples} I'll describe distributions over sequences that exhibit the bad modes problem in various ways, implying that even a model which was perfectly fit to that distribution would also have the bad mode problem.
Section~\ref{sec:modestheory_realistic} will argue that these distributions are not just theoretical, but may actually be present in real training data distributions.
While these results might seem to imply that we should give up on likelihood maximization altogether, Section~\ref{sec:modestheory_goodmodes} will describe situations which are mathematically identical to the bad mode problem, but instead the
\end{comment}

\section{Distributions with bad modes}\label{sec:modestheory_examples}
Model error is definitely a plausible partial cause of the results we went over in the previous section, and we won't be saying that NLG models are somehow free of error.
However, in this section we'll look at the exact modes of some sequence distributions, and see that they often have undesirable properties.
This has two implications: First, even if we could train error-free models, we'd still be stuck with the issue; and second, if we want to know that an outcome \emph{is} due to model error, we need to know that it isn't implied by the training data distribution.\footnote{For example, \citet{inadequacyofmode} compared the \emph{average} length of samples from their MT models to the average length of reference sentences from the data. They found some model error, but much less than one would assume from the empty mode results of \citet{catgotyourtongue}.}

If $\dtrain = \dclean$, then of course model error is implied by these results. 
However, we'll also show that adding relatively small amounts of noise to the data distribution can lead to $\dtrain$ having a bad mode.
It's not just ``garbage in, garbage out'', it's  ``tiny amount of garbage in, sizeable amount of garbage out.''

\subsubsection{Typicality}
A concept which is important for reasoning about these results is that of \emph{typicality}.
\citet{dieleman2020typicality} provides an excellent overview of the topic, and \citet{typical_sampling} applied the concept to NLG to come up with the \emph{locally typical sampling} method.
Informally, a typical sample is one that isn't much more or less likely to be observed than an average sample.
More formally, we'll call the typical set for a random variable $X \sim\mathcal{D}$:
\begin{equation}
    S = \left\{
        x\; \given[\big] \;
        \lvert
        -\log\prob_\mathcal{D} \left(X = x\right)
         - H(X)
        \rvert < \epsilon
    \right\}
\end{equation}
For some small $\epsilon$.
This is slightly different from the formulation used by \citet{typical_sampling}, since we want to compare sequences of different lengths on equal footing instead of normalizing by the length.

The bad mode problem is a particular example of atypicality: the mode is not a typical sample unless the distribution is extremely low entropy.
Frustratingly, we'll also see cases where atypicality is helpful, meaning we need to take a more nuanced view of when to try to find typical sequences.

\subsubsection{The bad mode problem}
We can now easily summarize the bad mode problem, and why it's counterintuitive.
Using the notation from Section~\ref{sec:modestheory_notation}:
\begin{equation}\label{eq:noncommutative}
    \argmax\limits_{a \in \mathcal{A}} \ptrain\left(A(X) = a\right) \neq A\left(\argmax\limits_{x \in \mathcal{S}} \ptrain(X = x)\right)
\end{equation}
I.e. the most likely attribute value is not the same as the attribute value of the most likely string.
If $A(x)$ is the indicator function of $\sclean$, this is just the bad mode problem: A distribution can have an arbitrarily high probability of yielding high-quality samples, but still have a low quality mode.
When the attribute is length, $A(x) = |x|$, then Equation~\ref{eq:noncommutative} says that the mode being empty doesn't imply anything about the modal length.

The rest of this section goes over cases where the lack of equality in Equation~\ref{eq:noncommutative} occurs.
This is often undesirable, but we'll also see cases where it's beneficial.

\subsection{Warm-up: Biased coin flips}\label{sec:coins}
This example comes from ~\citet{dieleman2020typicality} (originally from \citet{yung}).
Consider flipping a biased coin, which comes up heads 60\% of the time, 100 times.
(So $\seqs = \left\{H, T\right\}^{100}$).
Let $A$ be the function that counts the number of heads, so $\mathcal{A} = \{0, 1, \dots,100\}$.
The output of $A$ with the highest probability is 60, and there is an approximately 97\% probability that $50 \le A(X) \le 70$.
However, for a sequence with $N_H$ heads, the probability of observing that sequence is $(0.6)^{N_H}(0.4)^{100 - N_H}$, so the modal sequence consists entirely of heads.

This result is counterintuitive because grouping outcomes by the number of heads is natural to us, but the probability distribution doesn't care how we choose to partition it, it just assigns a weight to each of the $2^{100}$ outcomes.
Despite the counterintuitiveness, there's nothing objectively good or bad about this fact since we don't have any task or notion of quality to appeal to.
As such, this instance of atypicality is just a benign curiosity.

\subsection{Variable length sequences}\label{sec:modestheory_length}
Text generation is a good bit more complicated than flipping coins, so here we'll describe a distribution over sequences of variable length.
Predictably, we'll show that it's possible for the \emph{modal sequence} to be the empty sequence while the \emph{modal length} is arbitrarily high.

Let $\seqs$ be the regular language defined by $(a|b)*$, i.e. all finite strings consisting of one of two characters, including the empty string.
The attribute function will be the length $A(x) = |x|$.
Consider a random variable $X\in \seqs$ such that all strings of a given length have the same probability.
That is, for a length, $\ell$, $\prob(X = x | |x| = \ell)$ is the uniform distribution.
We'll write $p_\ell$ for the marginal probability that $X$ is length $\ell$.

The modal attribute value is the most common sequence length:
\begin{equation*}
\ell^* = \argmax\limits_\ell p_\ell
\end{equation*}

On the other hand, a modal sequence (there may be many) is defined by:
\begin{equation*}\label{eq:modes_length_argmax}
x^* = \argmax\limits_{x \in \seqs} \frac{p_{|x|}}{2^{|x|}}
\end{equation*}

For simplicity consider a strictly unimodal length distribution, i.e.:
\begin{align*}
    \ell < \ell^* &\implies p_\ell < p_{\ell + 1}\\
    \ell > \ell^* &\implies p_\ell < p_{\ell - 1}\\
\end{align*}
This implies that $|x^*| \le \ell^*$, since all the sequences longer than $\ell^*$ have lower probability than $p_{\ell^*}$.

If $p_\ell$ grows slowly enough, the right hand side of Equation~\ref{eq:modes_length_argmax} will be maximized when $\ell = 0$, implying that $x* = \epsilon$, the empty string.
The specific condition for this to be the case is:
\begin{align*}\label{eq:modes_length_bound}
   \frac{p_\ell}{p_0} < 2^{\ell}
\end{align*}
So, if the probability of a given output length grows less than exponentially quickly, the mode will be empty.
By using a sufficiently slowly growing sequence, $p_\ell$, one can have the length of the modal sequence arbitrarily high, while also having the empty sequence be modal.

This distribution is still extremely unrealistic, but it shows one facet of the issue: A single bad sequence with arbitrarily low quality can still have a higher likelihood than a high-entropy set of good or typical sequences.
We haven't defined a task (so there's no concept of $\sperfect$), but for all common NLG tasks, this outcome would be an instance of bad atypicality.

\subsection{Bland word choice}\label{sec:modestheory_templates}
Outputs which are too short is just the most obvious case of bad modes, but we can also construct distributions which have the problem while having constant length.
Here we'll let $seqs$ be instantiations of the template: \texttt{<name><vb.><adj.><noun>}, e.g. ``Joe eats delicious toast.''
For the distribution over $\seqs$:
\begin{itemize}
    \item For each slot, define a single common word which has probability 10\%, and 90 rare words which each have probability 1\%
    \item Each slot is filled independently
\end{itemize}
Now consider the attribute $A(x) = \text{\# of rare words in $x$}$.
The most common attribute value is $A(x) = 4$, since the probability of all four words being rare is $0.9^4 \approx 66\%$.
On the other hand, the modal string is made of the four common words, and has probability $1/10000$.

If we're interested in quality in the sense of representativeness or creativity, it's easy to see that this is a bad mode.
\citet{typical_sampling} argue that we should use locally typical sampling to achieve similar information content to natural text.
On this example, locally typical sampling would lead to outputs which have four rare words, which is representative of a typical output.

On the other hand, the mode actually globally maximizes BLEU score against a reference randomly sampled from this distribution.
If we look at this example as analogous to the choices a translation system needs to make in producing an output, our system would get a higher BLEU score by using the mode than a sampled output.
More importantly (maximizing BLEU isn't very motivating), what kind of translation we want likely depends on what the translations are for.
If every human translator injects their own personal flair or style into translation, we probably want to reflect that in translations of fiction or other works where rhetoric is important.
On the other hand, in translating technical documentation, a modal translation is probably fine, or even preferable, to one which is more natural.

In summary, if we want creativity and representativeness, the mode for this distribution is bad.
On the other hand, if we want outputs which are as ``standard'' as possible, the atypicality of the mode can even be beneficial.

\subsection{Independent errors}\label{sec:modestheory_errors}
Now we'll look at a case which is essentially the same as the previous example, but in this case, the atypicality will be desirable rather than harmful.

Consider a distribution over texts of in which first a text of $N$ sentences is sampled from some high quality distribution, $\dclean$.
Then, define $\dtrain$ as a distribution which takes samples from $\dclean$ introduces a typo into each sentence independently with probability $p_e$.

A typical text will contain $N p_e$ typos, but provided that $p_e$ is low enough, the most likely sequence should contain zero typos!\footnote{How low $p_e$ has to be depends on how likely typos which could have come from multiple different clean texts are.}
This is mathematically the same as Section~\ref{sec:modestheory_templates}, but with ``sentences with errors'' playing the role of ``rare words.''
The difference is just that in this case we want to avoid the ``rare'' phenomenon, rather than encouraging it.

So here, we have a type of atypicality which is (essentially) unambiguously good.
Representative examples from $\dtrain$ will have errors, and we want to avoid them!
Once noise is introduced, looking at outputs purely from an ``information-per-token'' or typicality point of view runs into some problems.
It isn't clear how to distinguish ``Low-probability because useful information is being added'' and ``Low-probability because there's a misspelling'' from the model probabilities alone.

\subsection{Summary}
We've shown several examples of sequence distributions which have modes unrepresentative of a typical sample.
Importantly, a perfectly trained model on any of these distributions would have a mode with the same property.
This means that observing these kinds of behaviors in a model is insufficient to demonstrate model error, unless you can also show that $\dtrain$ does not have that property.

This atypicality can be harmful, benign, or even helpful, depending on our aim.
Estimating statistics on samples drawn from the model, as \citet{inadequacyofmode} did, is the way to actually investigate approximation error.
Returning to the ``Oracle criterion'' from Section~\ref{sec:modestheory_notation}, it's clear that even given an oracle for the distributions in this section, MAP inference would be inappropriate for most of them.

However, sampling based approaches also wouldn't be able to clean up the errors in the noisy distribution from Section~\ref{sec:modestheory_errors}.
MBR decoding (using samples as hypotheses) and typical sampling would both output text with the average number of errors\footnote{MBR with the right cost function might reduce the number of errors, but once texts get long enough that all the hypotheses also have errors, the output will have errors as well.}
If we consider a distribution which suffers from both a bad mode \emph{and} noise in typical samples (as in the TV story at the beginning), it doesn't seem like any standard methods are up to the task.

\section{Modes of real data distributions}\label{sec:modestheory_realistic}
In this section we'll argue that two common NLG tasks, machine translation and chatbot instruction-following, might suffer from noise which leads to the presence of bad modes in their training data distribution.
$\sclean(x)$ for an MT input $x$ is the same as we said in Section~\ref{sec:modestheory_notation}: the set of valid translations of $x$ into the target language.
For the chatbot case $\sperfect(x)$ should only contain sequences which are ``good'' responses to the prompt $x$.

Since the definition of ``valid translation'' is a philosophical question, we can imagine operationalizing this with something like ``a panel of 5 UN translators would unanimously agree that $y$ is a faithful translation of $x$.''
For chatbots, the definition could be ``$y$ receives the maximum human rating on all criteria'' for some set of criteria such as being helpful and harmless.

If we got our training data from $\dperfect$, a model assigning non-zero probability to a low-quality text (i.e. one not in $\sclean$) would imply that there is model error present.
So the question is whether the the gap between $\dclean$ and $\dtrain$ for our actual training datasets is low enough for this conclusion to hold in practice.

Consider a specific model of $\dtrain$, which consists of samples from $\dperfect$ but with corruption randomly applied.
To say the training distribution has a bad mode for input $x$ means that there's some $y_\text{bad} \notin \sperfect$ such that:
\begin{equation*}\label{eq:bad}
    \ptrain\left(y_\text{bad} | x\right) \ge \max\limits_{y \in \sperfect} \ptrain(y | x)
\end{equation*}
It's hard to say anything specific about the right hand side of Equation~\ref{eq:bad} without any assumptions on $\ptrain$.
However, if we restrict our attention to outputs which are typical among the high-quality outputs, we can give an intuitive condition under which this will occur.

Write $\stypical(x)$ for the set of outputs $y$ which are typical \emph{high-quality} output for $x$.
$y\in \stypical(x)$ means that:
\begin{equation*}\label{eq:good_typical}
    \log \ptrain(y | x\; y\in\sperfect) \approx -\mathcal{H}_{\text{train}}(y | x,\; y\in\sperfect)
\end{equation*}
where $\mathcal{H}_{\text{train}}(\cdot | \cdot)$ is conditional entropy.
All values of $y$ which have an NLL similar to the conditional entropy will also have similar NLL to each other, so we can just think about the uniform distribution over the typical set.\footnote{The only reason we need to say have an approximate equality instead of equality anyways is because we're working with discrete random variables.}

We'll get either a bad or atypical mode when there's some $y \notin \sperfect(x)$ such that:
\begin{equation*}\label{eq:modes_uniform}
    \ptrain(y | x) > \frac{1}{|\stypical(x)|}
\end{equation*}
As we discussed in Section~\ref{sec:modestheory_related_work}, some version of ``number of valid responses'' is generally thought to be related to the bad mode problem appearing in practice as well.
For example, \citet{wiher2022ondecoding} found that for more ``directed tasks'' (i.e. ones with strong input-output relationships), deterministic decoding tended to work better; \citet{stahlberg2022uncertainty} used an edit-distance based metric as a proxy for measuring uncertainty, and found that MAP-type decoding was better for less uncertain tasks. Refer to Section~\ref{sec:modestheory_related_work} for a few more examples.

Equation~\ref{eq:modes_uniform} generalizes the reasoning from the length example in Section~\ref{sec:modestheory_length}.
To see the connection, consider the simplified case where for a given input $x$, all good outputs have the same length, and there's a bad output which has probability $p$ independent of the input.
Equation~\ref{eq:modes_uniform} says that this bad output could be modal if the entropy rate of the outputs of length $L$ ever exceeds $-\log p / L$.

There's no reason to think the output entropy rate decreases much with length for NLG tasks, other than maybe grammatical error correction.
\cite{catgotyourtongue} found that longer source sentences were \emph{more} likely to be assigned the empty sequence as a mode, which makes a lot of sense if MT has a constant output entropy rate!\footnote{MT doesn't have the guarantee that all translations of a source will be the same length, but they will generally be similar in length}

None of the above rules out model error though, since the above doesn't matter if $p = 0$ for all bad sequences.
We'll now look at some actual MT training data to see if that's the case.

\subsection{Empty sequences in Europarl}
Europarl~\citep{europarl} is a dataset of paired text from the European Parliament, widely used for training MT systems.
As of EuroParl-v7, the empty sequence is the most commonly occurring ``text'' in the English split of the German-English pair.
About 0.39\% of the 1.9 million paired sentences are a German text containing at least one alphabetical character and an empty English ``text.''
The median length in characters of these German texts is 35 characters, and the 90th percentile is 122.
Whatever the cause, the empty sequence is the empirical unconditional mode of this training corpus.

$\log_2 (1/0.0039) \approx 8$, meaning that if a typical high-quality sentence involves more than 8 binary decisions, the number of good translations will be too large for any one of them to be more likely than the empty sequence (on average).
Figure~\ref{fig:empty_europarl} shows the longest German sentence (884 characters long) which is paired with an empty English text.

Conservatively, imagine that all good translations of the German input are no more than 500 characters long.
A conditional entropy rate of even 0.04 bits per character\footnote{I.e. one binary decision per 25 characters} would require the probability of the empty sequence to be less than 1 in a million, or else it will dominate the good translations.

\begin{figure}
    \centering
    \small
    \begin{subfigure}{0.45\textwidth}
        \centering
        \fbox{\parbox{\textwidth}{``Ein solcher Basisbeschluß wird im Allgemeinen Rat gefaßt, so daß es sich - anders als es bei den Europäischen Räten sehr oft der Fall ist - um einen wirklich sorgfältig ausgearbeiteten und durchdachten Beschluß handelt, der dem Europäischen Rat unterbreitet wird; im Allgemeinen Rat kann anschließend im Rahmen eines solchen Basisbeschlusses ein Beschluß mit qualifizierter Mehrheit gefaßt werden, wobei wiederum für einen Mitgliedstaat die Möglichkeit besteht, einen solchen Beschluß anzufechten, wenn einem wichtigen nationalen Interesse dadurch geschadet wird; um zu verhindern, daß eine solche Anfechtung allzu häufig erfolgt, gilt ein Verfahren, wonach Zwei Drittel der Ratsmitglieder die Möglichkeit erhalten, beim Europäischen Rat Berufung einzulegen, damit ein letztes Urteil gefällt wird, wenn eine solche Anfechtung ihrer Ansicht nach zu unrecht erfolgte\texttt{</s>}''}}
        \caption{German source}
        \label{fig:empty_europarl}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \fbox{\parbox{\textwidth}{``\texttt{</s>}''}}
        \caption{English reference}
        \label{fig:subfigure2}
    \end{subfigure}
    
    \caption{A Europarl v7 De-En training example}
    \label{fig:figure}
\end{figure}

\subsection{Generalizing from truncation}
The clear objection at this point is that empty sequences should be filtered out during preprocessing.
If a model assigns a non-zero probability to the empty sequence in this case, there is definitely model error.
However, it could still be more appropriate to think of it as incorrect generalization.

Consider what's going on: Data is being sampled from a distribution which includes empty outputs, then being filtered to remove them.
Suppose you, the reader, were shown a training set of translations which included the following:
\begin{itemize}
\item German: ``Und der Liedtext geht weiter:'', English: ``And''.
\item German: ``(1) zur Hilfe der Europäischen Union für den Iran nach dem jüngsten Erdbeben'', English: ``(1)''
\end{itemize}
(These are also from Europarl, but it's much harder to estimate how much spurious truncation there is than it is to count how many empty English texts there are).

What betting odds would you be willing to take on a bet that the test set included precisely 0 empty outputs?
Very few people would put down even \$1,000 to win \$1, so their personal estimate of $\prob(\text{EOS})$ definitely can't be 0.
It shouldn't be too surprising that spurious EOS's sprinkled in the training data leads models to predict they might occur at the start of the sentence as well.

\citet{whynmtempty} conjectured that NMT models were oversmoothing due to a shared EOS token, and found that introducing per-position EOS tokens led to beam search producing empty outputs much less frequently.
This change makes it harder to make the incorrect generalization described above, and has the intended effect.

Besides the empty sequence problem, the examples above show we also need to worry about other types of degenerate translation.
Even if a model did put no probability on empty outputs, it may (correctly) have the modal output of producing a single word from a translation, \emph{then} EOS.
All the entropy-rate discussion from the previous sections applies to those types of outputs as well.

\subsection{Reinforcement learning-based instruction following}
In this section we'll give a sketch of how similar issues can arise even when training isn't done using MLE of the text distribution.

Consider a system like ChatGPT\footnote{\url{chat.openai.com}}, which is trained with Reinforcement Learning from Human Feedback (RLHF).
In this case, the model isn't being trained to fit any particular $\dtrain$, but the end result is still a distribution over sequences.
What should that distribution be?

One possible ideal distribution is the uniform distribution over all sequences which would get the maximum reward from the human raters.
RL doesn't actually elicit this distribution, since emitting a single output which receives maximal reward is easier and has the same expected reward.
Still, it's probably fair to say that a model which can give many different responses to ``Write a haiku'' is better than a model which just emits the same haiku every time.

One place noise can come from is incorrect human ratings, either due to misreading the text, or making data entry errors.
This is analogous to the corruption of $\dperfect$ discussed in the previous sections.

Just like with MT, we can come up with an input which has a high entropy output distribution.
Then we just have to show that there's a degenerate response with a negative log-likelihood lower than the entropy.

Consider the request ``Write a sonnet about NLP.''
Sonnets usually have around 100 words, so even at an extremely conservative entropy rate of 1 bit per word, there are $2^{100}$ valid responses, meaning we need to find a bad response which should have a probability higher than $1/2^{100}$.
One degenerate response is $y =$ ``I can't.''
Call the event that $y$ is maximally rated $R$, and the event that it's generated\footnote{by whatever distribution is being used to produce inputs to the rating process} $G$.
Then:
\begin{equation*}
    \prob(G | R) = \frac{\prob (R | G) P(G)}{P(R)}
\end{equation*}
The denominator on the right-hand side is at most 1, so the probability is bounded above by the numerator.
The numerator is just the product of the probabilities that ``$y$ is incorrectly given the maximal rating'' and ``$y$ is generated by the pre-RLHF model.''
In order for these probabilities to multiply to less than $2^{-100}$, one or both of them would need to be less than $2^{-50}$ (less than 1 quadrillionth).

Now, the ``equally probably outputs'' assumption isn't accurate for the current generation of chatbots.
On July 18, 2023, sampling outputs from GPT-4 for the above prompt 20 times led to 18 responses which started with ``Upon'', with the other two starting with ``In the realm.''
``Realm'' appears in the first line of 7 out of 20 responses. We'll look at modal outputs for some open source instruction-following chatbots in Chapter~\ref{chapter:modes_exact}, and show that this behavior is present in them as well.

So maybe beam search or other MAP approximations \emph{would} work well on these models, since their output entropy is so much lower than the ideal distribution.
We probably do want to produce better chatbots over time though, so the entropy of their outputs will necessarily rise (at least for certain inputs).

\section{Implications}\label{sec:modestheory_proposal}
Getting back to the ``oracle criterion'' again, it's doesn't seem like any common decoding method would consistently give us good samples from an oracle for $\ptrain (y_t | x, y_{1:t-1})$.
If the training distribution contains low-quality/low-entropy outputs (e.g. the empty sequence, ``I don't know'', ``As an AI language model, I cannot...''), then likelihood maximization strategies will fail.
On the other hand, if a typical sample is corrupted by a small amount of noise, sampling-based methods will also produce outputs with the same amount of noise.

The problem is at least partly that likelihood alone doesn't let us distinguish between low-probability but meaningful information, and low-probability noise such as typos.
As far as the distribution is concerned, they're both high-information!
Similarly, it can't let us distinguish between text which is high-probability because it is relevant to the input, and text which is high-probability because the distribution has low-quality modes.

At the very least, if you find the examples above convincing, don't conclude that your model learned the data poorly just because it outputs some low-quality text.
To assess whether a model has learned the distribution, you should draw samples from it and measure their statistics, as done by \citet{inadequacyofmode}.
You might need to use evaluations of single outputs for practical reasons, but it's important to view the results as a combined evaluation of \emph{both} the model and a decoding strategy.

For convenience we'll repeat Equation~\ref{eq:noncommutative} here:
\begin{equation*}
    \argmax\limits_{a \in \mathcal{A}} \prob\left(A(X) = a\right) \neq A\left(\argmax\limits_{x \in \mathcal{S}} P(X = x)\right)
\end{equation*}
We said before that the non-intuitive behavior of non-typical outputs is because these two quantities aren't equal.
The right hand side is what we're seeing when a model's mode is the empty sequence, and the left hand side is what we're seeing when a sampling-based method spits out noise at the same rate as it was present in the training data.

But this suggests a way to improve our decoding outputs, we can just condition on the argmax value from the left-hand-side of Equation~\ref{eq:noncommutative}.
Imagine translating this thesis into German, and call $l^*$ the modal translation length (\emph{not} the length of the mode).
$l^*$ is definitely greater than 10,000 but the modal translation would be much shorter (or even empty), due to the entropy rate issue discussed previously.
Instead of searching for the argmax translation $x \in \seqs$, we should be looking for the conditional argmax:
\begin{equation*}\label{eq:cond_mode}
    x_\text{cond}^* = \argmax\limits_{x \in \seqs} \prob \left( X = x \given[\big] |x| = l^*\right)
\end{equation*}
This is actually already common in another setting, although it's not usually framed this way.
Non-autoregressive (Non-AR) NMT systems usually \emph{have} to do this because of their architecture.
For example, SUNDAE~\citep{sundae} predicts the length of the target sentence from the source sentence, then searches for a high scoring sequence \emph{of that length}.
If someone suggested trying to maximize the product $\prob(\text{length}) \prob(X | \text{length})$ in that setting, everyone would think they were crazy!
This might partially explain why short outputs are often seen as a bias of autoregressive models.
Non-AR models avoid the problem by construction!

To avoid degeneracies other than brevity, we could imagine conditioning on other attributes as well.
If the modal response from a chatbot is ``I don't know'', it would be much more interesting to find the modal response \emph{conditional on attempting to reply}.

A reasonable question is whether this will actually give us good outputs, or if we'll just be patching up an endless sequence of failure modes.
For example, maybe the modal length-20,0000 translation of this thesis is just the word ``NLG'' repeated 20,000 times.
In the next chapter, we'll look at some exact length-conditional modes of a pretrained NMT model and see that they're actually pretty high quality!

Since finding exact modes is expensive, if not intractable, in Chapter~\ref{chapter:modes_beam} we'll propose a beam search variant which can be used for search conditional on an attribute.
It doesn't just work for controlling length in MT, but also for applying beam search to an open domain LM.
We aren't proposing that writing a sonnet with MAP decoding is a good idea, but for settings where correctness is important, there's a lot to be gained by being able to do some sort of likelihood maximization.
The idealized end-goal of this line of research would be to decode from the conditional probability $\prob\left(x\given x\text{ is not degenerate}\right)$.

We should also point out that the ``attribute of mode does not equal modal attribute'' problem also suggests another solution.
If sampling-based repeats noise from the training distribution, you could for example sample from the conditional probability $\prob(x \given x\text{ is fluent})$.
More ambitiously, you could even consider sampling from $\prob(y \given x,\;\text{$y$ is a translation of $x$})$.
The idealized final result for RLHF training of LMs would be to directly sample from $\prob(y \given x,\; y\text{ is high-reward})$.

Sampling from conditional distributions has been researched before, although the conditioning information is generally things like topic or sentiment.
The most relevant method is FUDGE, which uses a classifier which predicts the final value of an attribute given a partial model output.
The way to use FUDGE for this particular task would be to train a classifier to predict the total number of typos in the output, or whether the final output will be a valid translation of the source sentence given the output so far.

Basically, we're suggesting using search on $\prob ( x | \text{$x$ is not degenerate})$, or sampling on $\prob (x | \text{$x$ is correct/not noisy})$.
Of these two options, we'll be focusing on search over sampling.
The first reason is that search (especially for language models) has received less attention than sampling, so we expect that there's more room for improvement.
Secondly, the relevant problem for fixing MAP degeneracies is predicting things like ``will the output be empty'' or ``does the output attempt to fulfill the prompt'', which we expect to be much easier to learn than ``will the output be factual.''
That being said, we hope that future work will investigate sampling from these conditional distributions.

\section{Conclusion}
The main point of this chapter has been to convince you that many observed degeneracies in NLG \emph{could} be due to properties of the training data distribution, rather than directly implying model error.
We described noise models for both MT data and RLHF trained LMs which would lead to these phenomena being present even in realistic settings.

Our decoding methods need to take this into account, since we'll be stuck with the issue unless we manage to only train on extremely clean data.
Our proposed path forward is to explicitly incorporate more information about the properties we want in our decoding outputs, rather than using methods which only depend on model likelihood.

\begin{comment}
\subsection{Reinterpretations}
Cat got your tongue
This is not incorrect, as it's true that the procedure ``use MAP decoding on an NMT model'' produces empty sequences far more than the training data would indicate.
This is \emph{not} the same that claiming the learned NMT model underestimates the average length, which for a translation $Y$ of source $X$ would be:
\begin{equation}\label{eq:modes_expected_length}
     E_{Y\sim \dmodel} [|Y| \given X] < E_{Y~\sim \dpop} [|Y| \given X]
\end{equation}
We will make a more general point about this kind of distinction later on.

Likelihood-Utility
This taxonomy correctly points out many sources of error, but we will discuss cases where the quality-likelihood divergence can occur without any of these being present.
In Section~\ref{sec:modes_examples} we will discuss individual sequence distributions with good samples but bad modes, meaning that the issue cannot be due to any sort of drift or approximation error.

\subsection{Other related work stuff}
\citet{typical_sampling}
\paragraph{Findings:} Following the idea that ``per-unit information content'' a factor in how human-like text is, the authors propose \emph{locally typical sampling} (LTS).
LTS is a decoding method which samples from tokens which have a conditional log-probability close to the average log-probability of the next-token distribution (i.e. its conditional entropy).
LTS seems to qualitatively outperform the other sampling methods, but beam search is still slightly better in terms of performance on abstractive summarization, despite being less human-like.
\paragraph{Interpretation:} The authors 
\end{comment}

==> new_appendices/beam_search_derivation.tex <==
\section{Derivation of conditional beam search update}

\begin{align}
    S'(x_{1:t}, a) &= \sum\limits_{i=1}^t \log P(x_i | x_{<i}, a)\\
    &= \sum\limits_{i=1}^t \log \frac{P(a | x_{\le i})P(x_i | x_{<i})}{P(a | x_{<i})}\\
    &= \left(\sum\limits_{i=1}^t \log P(x_i | x_{<i})\right) + \sum\limits_{i=1}^t \log\frac{P(a | x_{\le i})}{P(a | x_{<i})}\\
    &= S(x_{1:t}) + \log\frac{P(a | x_{\le t})}{P(a | x_{<1})}\\
    &= S(x_{1:t}) + \log\frac{P(a | x_{\le t})}{P(a )}\\
\end{align}

==> new_appendices/cond_beam_search_algorithm.tex <==
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}
\begin{algorithm}
\caption{Conditional beam search. This searches for an output with a sequence $x$ with a high value of $\pmodel(x, A(x) = a)$ for some target attribute $a$. In order to execute this efficiently one needs to efficiently compute $\pmodel$ and $\pclf$ to avoid recomputation. This will typically involve caching transformer hidden states, as is standard for causal transformers.}\label{alg:beam_cond}
 \hspace*{\algorithmicindent}\textbf{Input:} \\
 \hspace*{\algorithmicindent} $\: a$: The target attribute value\\
 \hspace*{\algorithmicindent} $\: V$: Vocabulary\\
 \hspace*{\algorithmicindent} $\: B > 0$: Beam size\\
 \hspace*{\algorithmicindent} $\: L > 0$: Maximum output length\\
 \hspace*{\algorithmicindent} $\: k > 0$: Number of continuations to score for each hypothesis.\\
 \hspace*{\algorithmicindent} $\: \alpha > 0$: Optional attribute weight.\\
 \hspace*{\algorithmicindent}\textbf{Output:} A string in $V*$ with length at most $L$
\begin{algorithmic}[1]
\State $X[b] = \epsilon$ for $b \in {1, \dots, B}$ \qquad\{Initialize all hypotheses to the empty sequence\}
\State $S \gets [0, -\infty, -\infty, \dots, -\infty]$ \qquad\{A length $B$ array of cumulative scores, only $S[0]$ is initially finite.\}
\State $t \gets 1$
\While{Any hypothesis $X[i]$ on the beam is not complete AND $t \le L$}
    \State Init empty $b \times k$ array $U_t$ \qquad\{Unconditional scores\}
    \State Init empty $b \times k$ array $C_t$ \qquad\{Conditional scores)\}
    \State Init empty $b \times k$ array $C'_t$ \qquad\{Weighted conditional scores, optional\}
    \State Init empty $b \times k$ array $W$ \qquad\{Continuations\}
    \For{$b = 1, \dots, B$}
        \If {$t < L$}
            \State $L[w] \gets \log\pmodel (w | x_{1:t} = X[b])$ \{for all $w \in |V|$\}
        \Else
            \State $L[:] \gets -\infty$
            \State $L[\text{\tt </s>}] \gets 0$ \qquad\{If at the max sequence length, all hypotheses are forced to be complete\}
        \EndIf
        \State $W[b, :] \gets$ words with top $k$ scores in $L$
        \For {$i = 1, \dots, k$}\qquad{}
            \State $w \gets W[b, i]$
            \State $U_t[b, i] \gets S[b] + L[w]$
            \State $C_t[b, i] \gets U[b, :] + \log\pclf(a | x_{t+1} = w, x_{1:t} = X[b])$
            \State $C'_t[b, i] \gets U[b, :] + \alpha\log\pclf(a | x_{t+1} = w, x_{1:t} = X[b])$
        \EndFor
    \EndFor
    \State \{We select new beam elements using $C'_t$, but update $S$ using $U_t$.\}
    \For{$b = 1, \dots, B$}
        \State $b_\text{prev}, i \gets$ $b$-th largest pair of indices into $C'_t$
        \State $S[b,i] \gets U_t[b_\text{prev}, i]$
        \State $X[b] \gets \mathrm{concatenate}\left(X[b_\text{prev}], W[b_\text{prev}, i]\right)$
    \EndFor
\EndWhile
\If {Attribute is deterministic}
    \State $b_\text{best} = 1$
\Else
    \State $b_\text{best} \gets \argmax\limits_{i} C_t[i]$\qquad\{If the classifier is uncertain about the value of the attribute even for a complete output, we take that into account when selecting the output.\}
\EndIf
\State \textbf{Return} $X[b_\text{best}]$
\end{algorithmic}
\end{algorithm}
